A Quantum Approximate Optimization Method For Finding Hadamard Matrices

Finding a Hadamard matrix of a specific order using a quantum computer can lead to a demonstration of practical quantum advantage. Earlier efforts using a quantum annealer were impeded by the limitations of the present quantum resource and its capability to implement high order interaction terms, which for an $M$-order matrix will grow by $O(M^2)$. In this paper, we propose a novel qubit-efficient method by implementing the Hadamard matrix searching algorithm on a gate-based quantum computer. We achieve this by employing the Quantum Approximate Optimization Algorithm (QAOA). Since high order interaction terms that are implemented on a gate-based quantum computer do not need ancillary qubits, the proposed method reduces the required number of qubits into $O(M)$. We present the formulation of the method, construction of corresponding quantum circuits, and experiment results in both a quantum simulator and a real gate-based quantum computer.

==> 2_1__HSEARCH.tex <==
\subsection{Finding H-Matrices as a Binary Optimization Problem}

A direct method to find an $M$-order a H-matrix, i.e. a binary orthogonal matrix of size $M\times M$, can be done by checking the orthogonality condition of all possible binary matrices $B=[b_{m,n}]$, where $b_{m,n} \in \{-1, +1\}$. The orthogonality test can be formulated as a cost function $C_D(B)$, which is the sum of the squared off-diagonal elements of an indicator matrix $D=[d_{m,n}]=B^TB$, which can be expressed by, 
\begin{equation}
    C_D(B) = C(b_{m,n}) = \sum_{m=0}^{M-1} \sum_{n=0}^{M-1} \left(d_{m,n}- I_{m,n} \right)^2  
\end{equation}
%
where $I$ is an $M\times M$ identity matrix. When $C_D(B)=0$, then the matrix $B$ is orthogonal and therefore it is a H-matrix; otherwise it is not. It is not an efficient method due to the number of binary matrices to check is $2^{M\times M}$. 

A more efficient way of finding the H-matrix is by employing the Williamson/Baumert-Hall \cite{hedayat_1978} or the Turyn methods \cite{turyn_1974, kharaghani_rezaie_2004, london_2013}. We also have developed optimization based methods that employs quantum computers to find the H-matrix, which are the QA (Quantum Annealing) direct method by representing each entries as a binary variable \cite{suksmono_minato_2019}, the QA Williamson/Baumert-Hall method, and the QA Turyn method \cite{suksmono_2022}. Whereas the number of variables in the QA direct method grows with the order $M$ by $O(M\times M)$, the QA Williamson/Baumert-Hall and the QA Turyn methods only grows by $O(M)$, which is more efficient in term of the number of the variables. However, when it is implemented on the present day quantum annealer, such as the D-Wave, not only each variable should be represented by a qubit, but additional \emph{ancillary} qubits are also required for representing  3-body and 4-body terms. Accordingly, the required number of qubits grows with the order of the matrix by $O(M\times M)$. Since the qubit is one of the most valuable resources in quantum computing, a more efficient method that can reduce the number of qubits is highly desired.

In the Williamson based method \cite{suksmono_2022}, we seek for a binary $\{-1, +1\}$ vector
\begin{equation}
   \vec{s}=\left[s_0, s_1, \cdots, s_n, \, \cdots, s_{N-1} \right] 
   \label{EQ_WBH_string}
\end{equation}
%
where $s_n \in \{-1,+1\}$, that minimize a Williamson cost function $C_W(\vec{s})$ that is given by,
%
\begin{equation}
    C_W(\vec{s}) = \sum_{i=0}^{K-1} \sum_{j=0}^{K-1} \left(v_{i,j}(\vec{s})- 4k\delta_{i,j}\right)^2
    \label{EQ_cost_williamson}
\end{equation}
% 
In this equation, $v_{i,j}(\vec{s})$ is the elements of matrix $V$ that is constructed from four sub-matrices $A,B,C, $ and $D$ of dimension $K \times K$; that is,
%
\begin{equation}
    V = A^TA + B^TB + C^TC +D^TD    
\end{equation}
%
where $V=V(\vec{s}), A=A(\vec{s}), B=B(\vec{s}), C=C(\vec{s}), D=D(\vec{s})$ are sub-matrices whose elements include some particular elements of the vector $\vec{s}$. When $C_W(\vec{s})=0$, then the matrix $H$ of size $4K \times 4K$ given by the following block matrix
\begin{equation}
    H = 
    \begin{pmatrix}
        A & B &  C & D \\
       -B & A & -D & C \\
       -C & D &  A &-B \\
       -D &-C &  B & A
    \end{pmatrix}
\end{equation}
is Hadamard \cite{hedayat_1978}. A larger Baumert-Hall matrix can also be constructed from the same $\{A, B, C, D\}$ submatrices \cite{hedayat_1978}. We will call the binary representation of vector $\vec{s}$ given in Eq. (\ref{EQ_WBH_string}) that minimize Eq.(\ref{EQ_cost_williamson}) as a Williamson/Baumert-Hall string or a \emph{WBH-string}.

%////////////////////////////////////////////
% INCLUDE ... ???
%////////////////////////////////////////////
In the Turyn based method, we also seek for a vector $\vec{s}=[s_0, s_1, \cdots , s_{N-1}]$ like in Eq.(\ref{EQ_WBH_string}) that minimize a Turyn cost function $C_T(\vec{s})$ given by
\begin{equation}
    C_T(\vec{s}) = \sum_{r>1} \left( N_{X(\vec{s})}(r) + N_{Y(\vec{s})}(r) + 2N_{Z(\vec{s})}(r) + 2N_{W(\vec{s})}(r) \right)^2
    \label{EQ_cost_turyn}
\end{equation}
%
where $N_{X(\vec{s})}(r), N_{Y(\vec{s})}(r), N_{Z(\vec{s})}(r), N_{W(\vec{s})}(r)$ are non-periodic auto-correlation functions of sequences $X(\vec{s}), Y(\vec{s}), Z(\vec{s}), W(\vec{s})$, respectively, which are calculated at lagged $r$. Note that for a sequence $X=[x_0, x_1, \cdots, x_{N-1}]$, the non-periodic auto-correlation function is given by \cite{kharaghani_rezaie_2004, london_2013},

\begin{equation}
N_X(r) = 
     \begin{cases}
       \sum_{n=0}^{N-1-r} x_n x_{n+r} &, 0 \leq r \leq N-1\\
       0 &, r \ge N\\
     \end{cases}
\end{equation}
%
Similarly as in the previous case, we will call the bianry representation of vector $\vec{s}$ that makes $C_T(\vec{s})=0$ as a Turyn string or \emph{T-string}. In this paper, since the number of variables can be very large, the computation of the cost functions $C_W(\vec{s})$ and $C_T(\vec{s})$ and its corresponding Hamiltonian expression are performed by symbolic computing.



==> 2_2__QAOA_HSEARCH.tex <==
%\subsection{A Brief on QAOA}
\subsection{QAOA Formulation of H-matrix Searching Problem}
%% Section 2.2 dan 2.3 perlu disatukan dng judul section spt di atas
%\subsection{A Brief on QAOA (Quantum Approximate Optimization Algorithm)}
%%%//////////////////////////////////////////////////
% this part of qaoa formulation/derivation
% from time-dependent schrodinger SHOULD BE
% verified with standard book/paper, such as Farhi's
%%%//////////////////////////////////////////////////
 
%Present days quantum computers are categorized as NISQ (Noisy Intermediate Scale Quantum) devices, which means that the qubits are noisy and the number of qubits is not sufficiently large ($< 1000$)\cite{preskill_2018}. To harness its capability, various quantum algorithms that works on NISQ devices are developed. Among others is the QAOA (Quantum Approximate Optimization Algorithm) proposed by Farhi \cite{farhi_2014}. 

%Most recently, Kim et.al \cite{kim_2023} showed an evidence of the utility of NISQ device without fault tolerance qubits

%%%--Most recently, Kim et.al \cite{kim_2023} showed an evidence of the utility of NISQ device without fault tolerance qubits.

%The time-dependent Schroedinger Equation for a quantum system with Hamiltonian $H$ is given by
%\begin{equation}
%    i\hslash \frac{\partial \ket{\psi_t}}{\partial t} = H\ket{\psi_t}
%\end{equation}
%with a general solution
%\begin{equation}
%    \ket{\psi_t} = e^{-i\frac{Ht}{\hslash}}  \ket{\psi_0} = U(H,t)\ket{\psi_0}
%\end{equation}
%with unitary evolution given by
%\begin{equation}
%    U(H,t)=e^{-i\frac{Ht}{\hslash}}
%  \label{EQ_unitary}
%\end{equation}
%%//// tentative after this, ref to 
%// https://pennylane.ai/qml/demos/tutorial_qaoa_intro//
%
% H=H_1+H_2 + ... +H_n
% with H_i noncommutative in general. We can approximate using trotter-Suzuki decomposition formula
%\begin{equation}
% e^{H_i + H_j} \approx \left( e^{\frac{H_i}{n} e^{\frac{H_j}{n}} \right) ^n 
%    \label{EQ_trotter_suzuki}
%\end{equation}
%The unitary can be approximated with $n$-time step discretization as follows
%\begin{equation}
%    \nonumber
%    U(t, t_0) \approx U(t,t_n)U(t,t_{n-1}) \cdots U(t_1,t_0)
%\end{equation}
%and by using \ref{EQ_unitary}, we have
%\begin{equation}
%    \nonumber
%    U(t, t_0) \approx e^{-i\frac{H_n(t-t_n)}{\hslash}}
%    e^{-i\frac{H_{n-1}(t_n-t_{n-1})}{\hslash}} \cdots
%    e^{-i\frac{H_1(t_1-t_0)}{\hslash}}
%\end{equation}

%The QAOA is a quantum algorithm to approximate a solution of a combinatorial optimization problem that can work on the NISQ devices. It works as follows.

The QAOA is a hybrid classical-quantum algorithm proposed by Farhi et.al \cite{farhi_2014}.  It is a solution for near-term quantum computing, which can be implemented on a Noisy Intermediate-Scale Quantum (NISQ) device; i.e., a quantum computer with limited number of qubits, connectivity,  gate errors,  and short coherence times. A typical $N$-bit and $M$-clause combinatorial optimization problem addressed by the QAOA can be formulated as follows.  Consider an $N$-length bit string $\vec{b}=b_0b_1 \cdots b_{N-1}$ and let $C(\vec{b})$ be a cost or an objective function given by the following expression
%
\begin{equation}
    C(\vec{b}) = \sum_{m=0}^{M-1} C_m(\vec{b})
    \label{EQ_QAOA_basic}
\end{equation}
%
The value of $C_m(\vec{b})$ is equal to 1 if $\vec{b}$ satisfies the clause $C_m$, otherwise it is $0$ . When $C$ is the maximum value of Eq. (\ref{EQ_QAOA_basic}), the approximation means that we seek for a bit string $\vec{b}$ where $C(\vec{b})$ is close to $C$.

%Alternatively, 
For applying the QAOA to the H-matrix searching problem, we change the Boolean vector $\vec{b}$ in Eq. (\ref{EQ_QAOA_basic}) into into its spin vector representation $\vec{s}=[s_0, s_1, \cdots, s_M]$, while the maximization is recast as minimization. We can restate the previous approximation problem into finding a vector $\vec{s}$ that minimize a non-negative cost function given by

\begin{equation}
    C(\vec{s}) = \sum_{m=0}^{M-1} C_m(\vec{s})
    \label{EQ_QAOA_spin}
\end{equation}
%
Then, the approximation means that we seek for a bit string $\vec{b}$ corresponding to the vector $\vec{s}$ that makes $C(\vec{s})$ close to zero. %Such a binary string $\vec{b}$ that makes $C(\vec{b})=C$ or a spin vector $\vec{s}$ that makes $C(\vec{s})=0$ is called a \emph{valid string}. %???????

In the QAOA method, we have a Hamiltonian $H$ that consists of a \emph{problem Hamiltonian} $H_C$ and a \emph{mixer Hamiltonian} $H_B$,
%
\begin{equation}
    H = H_C + H_B
\end{equation}
%
Then, we construct a quantum circuit to perform the following unitary transform  
\begin{equation}
      U(\gamma, \beta) = e^{-i\beta_P H_B}e^{-i\gamma_P H_C} e^{-i\beta_{P-1} H_B}e^{-i\gamma_{P-1} H_C} \cdots e^{-i\beta_p H_B}e^{-i\gamma_p H_C}  \cdots e^{-i\beta_1 H_B}e^{-i\gamma_1 H_C}
    \label{EQ_QAOA_general}%
\end{equation}
where
\begin{equation}
  H_B=\sum_j b_j \hat{\sigma}^x_j  
  \label{EQ_QAOA_driver}%
\end{equation}
and
\begin{equation}
    H_C=\sum_{j,k, \cdots,m,n} c_{jk\cdots mn} \hat{\sigma}^z_j\hat{\sigma}^z_k\cdots \hat{\sigma}^z_m\hat{\sigma}^z_n  
  \label{EQ_QAOA_problem}%
\end{equation}
%    H_C=\sum_{j,k, \cdots,m,n} c_{j,k,\cdots, m,n} \sigma^z_j\sigma^z_k\cdots \sigma^z_m\sigma^z_n  
In these equations, $P$ is the number of layers (Trotter slice),  $\gamma_p$ and $\beta_p$ are  (angle) parameters at layer $p$, $b_j$ and $c_{j,k,\cdots, m,n}$ are constants, whereas $\hat{\sigma}^x_j$ and $\hat{\sigma}^z_j$ are the $j^{th}$ spin/Pauli matrices in $x$ and $z$-directions, respectively.

The term expressed by the product of $n$ Pauli matrices $\hat{\sigma}_0^z\hat{\sigma}_1^z \cdots \hat{\sigma}_{n-1}^z$ in Eq.(\ref{EQ_QAOA_problem}) is called an $n$-body interaction term. In the Hadamard Searching Problem (H-SEARCH), there are only up to 4-body interaction in the Hamiltonian, so that generally $H_C$ can be expressed by

\begin{equation}
    H_C=\sum_{j} c_j \hat{\sigma}^z_j  +
    \sum_{j,k}c_{jk}\hat{\sigma}^z_j\hat{\sigma}^z_k +
    \sum_{j,k,m} c_{jkm} \hat{\sigma}^z_j\hat{\sigma}^z_k\hat{\sigma}^z_m + 
    \sum_{j,k,m,n} c_{jkmn} \hat{\sigma}^z_j\hat{\sigma}^z_k\hat{\sigma}^z_m\hat{\sigma}^z_n 
  \label{EQ_QAOA_problem_hsearch}%
\end{equation}
%
%In the followings, we will describe how to construct quantum circuits related to each of the $n$-body interactions. % and present an example of finding a 2-order H-matrix.
%%%%%%%%%%%%%
%\subsection{Construction of Quantum Circuits with $n$-body Interaction}
% for 1-body, 2-body, 3-body, and 4-body interactions
%
The construction of quantum circuits related to each term of the $n$-body interactions in Eq.(\ref{EQ_QAOA_problem_hsearch}) are done as follows.

Consider a general problem Hamiltonian given by Eq. (\ref{EQ_QAOA_problem_hsearch}). By using Eq.(\ref{EQ_QAOA_general}), the unitary for of a single layer problem's Hamiltonian can be expressed by
\begin{equation}
    \label{EQ_problem_h_unitary}
    U(\gamma)=\prod_{j}e^{-i\gamma c_j\hat{\sigma}^z_j}
            \prod_{j,k}e^{-i\gamma c_{jk}\hat{\sigma}^z_j\hat{\sigma}^z_k}
            \prod_{j,k,m}e^{-i\gamma c_{jkm}\hat{\sigma}^z_j\hat{\sigma}^z_k\hat{\sigma}^z_m}
            \prod_{j,k,m,n}e^{-i\gamma c_{jkmn}\hat{\sigma}^z_j\hat{\sigma}^z_k\hat{\sigma}^z_m\hat{\sigma}^z_n}
\end{equation}
%e^{-i\gamma H_C}=
%
% -- 1-Body ------
%\begin{figure*}[h!]
%    \centering
%    \subfloat[\centering 1-body interaction]
%    {{\includegraphics[width=0.45\columnwidth]{img/1_body.jpg} }}% 
%    %\qquad
%    \subfloat[\centering 2-body interaction]
%    {{\includegraphics[width=0.45\columnwidth]{img/2_body.jpg} }} %
%    %\hspace{1}
%    \\
%    %\\
%    \subfloat[\centering 3-body interaction]
%    {{\includegraphics[width=0.6\columnwidth]{img/3_body.jpg} }}%
%    \\
%    %\qquad
%    \subfloat[\centering 4-body interaction]
%    {{\includegraphics[width=0.8\columnwidth]{img/4_body.jpg} }}%
%    %%%
%    \caption{Quantum Circuits for 1-,2-,3-, and 4-body interaction terms in the Hamiltonian}%
%    \label{FIG_1BODY}%
%\end{figure*}

\begin{figure}[h!]
    \centering
    \includegraphics[width=1.0\columnwidth] {img/qc_elements_12_44} 
    \caption{Elementary and QAOA-Implemented Quantum Circuits: (a) 1-body term, (b) 2-body term, (c) 3-body term, (d) 4-body-term, (e) a 1-layer quantum for 12-order QAOA-Williamson/Baumert-Hall method, and (f) a 1-layer quantum circuit of 44-order QAOA-Turyn method.} %  (g) an instance of 127 qubits arrangement in IBM-Brisbane Eagle processor, and (h) a photograph of 127 qubits Eagle quantum chip//When $P_x > P_R$, then the x-algorithm is considered useful.}
    \label{FIG_1BODY}
\end{figure}
%
We can represent the exponentiation of $\hat{\sigma}^z$ as a rotation in $z$-direction, $R_Z(\cdots)$, as  follows
\begin{equation}
    \nonumber
     U(\gamma) = e^{-i\gamma \hat{\sigma}^z} 
     = e^{-i\gamma 
     \begin{pmatrix}
      1 & 0 \\
      0 & -1
     \end{pmatrix}
     }
     =  
     \begin{pmatrix}
      e^{-i\gamma} & 0 \\
      0 & e^{i\gamma}
     \end{pmatrix}
     = R_Z(2\gamma)
\end{equation}
%
By substitution of $\gamma' = c_j \gamma$, we  have
\begin{equation}
    \nonumber
     U(c_j\gamma)=U(\gamma') = e^{-c_j\gamma \hat{\sigma}^z} = R_Z(2c_j\gamma)
\end{equation}
%
The first term of the product in Eq.(\ref{EQ_problem_h_unitary}), considering there are $N$ qubits to be rotated, can be expanded into

\begin{equation}
    \nonumber
    \prod_{j} e^{-ic_j\gamma \hat{\sigma}_j^z} =  
    \begin{pmatrix}
      e^{-ic_0\gamma} & 0 \\
      0 & e^{ic_0\gamma}
    \end{pmatrix}
    \otimes
    \begin{pmatrix}
      e^{-ic_1\gamma} & 0 \\
      0 & e^{ic_1\gamma}
    \end{pmatrix}
    \otimes
    \cdots
    \otimes
    \begin{pmatrix}
      e^{-ic_{N-1}\gamma} & 0 \\
      0 & e^{ic_{N-1}\gamma}
    \end{pmatrix}
    %\label{EQ_unitary_1body_prod}
\end{equation}
or, by denoting the $Z$ rotation on qubit $n$ as $R_{Z_n(\cdots)}$, we can write
\begin{equation}
    \nonumber
    \prod_{j} e^{-ic_j\sigma_j^z} 
    = R_{Z_0}(2c_0\gamma) \otimes R_{Z_1}(2c_1\gamma) \otimes \cdots \otimes R_{Z_{N-1}}(2c_{N-1}\gamma)
    \label{EQ_unitary_1body_prod}
\end{equation}
%
%%%%% //// 
The products in Eq.(\ref{EQ_problem_h_unitary}) can be interpreted as a cascaded operations. Then, a 1-body terms in the Hamiltonian that is expressed by $H_{C1}= \sum_j c_j \hat{\sigma}^z_j$ can be implemented as a quantum circuit given by Fig. \ref{FIG_1BODY}.(a), which is a Z-rotation of angle $2c_j\gamma$.
%\begin{equation}
%    H_{C1}= \sum_j c_j \sigma^z_j
%\end{equation}
%
Higher order terms, which are 2-,3-, and 4- body interacting terms, can also be treated similarly, but with a different elementary circuits in the cascaded block. 

The quantum circuits implementation of the $k$-body interactions displayed in Fig. \ref{FIG_1BODY} (b), (c), and (d) are adopted from Nielsen-Chuang \cite{nielsen_chuang_2010}, Seeley \cite{seeley_2012}, and Setia \cite{setia_2018}. A 2-body terms in the Hamiltonian $H_{C_2}= \sum_{j<k} c_{jk}\hat{\sigma}^z_j\hat{\sigma}^z_k$ has a corresponding circuits given by Fig. \ref{FIG_1BODY}.(b), which is a combination of CNOT and Z-rotation gate. The 3-body terms in the Hamiltonian which is expressed by $H_{C_3}= \sum_{j<k<m} c_{jkm} \hat{\sigma}^z_j\hat{\sigma}^z_k\hat{\sigma}^z_m$ has a corresponding circuits given by Fig. \ref{FIG_1BODY}.(c), which is a combination of CNOT and Z-rotation gate acting on 3 qubits. Finally, a 4-body terms in the Hamiltonian  $H_{C_4}= \sum_{j<k<m<n} c_{jkmn} \hat{\sigma}^z_j\hat{\sigma}^z_k\hat{\sigma}^z_m\hat{\sigma}^z_n$ has a corresponding circuits given by Fig.\ref{FIG_1BODY}.(d), which is a combination of CNOT and Z-rotation gate acting on 4 qubits. This figure also display a 1-layer quantum circuit of 12-order QAOA WBH and 44-order QAOA Turyn methods constructed from 1-, 2-, 3-, and 4- body terms circuits; displayed in (e) and (f) respectively, which will be discussed in more detail in the following sections. 

%\begin{equation}
%    H_{C2}= \sum_{j<k} c_{jk}\sigma^z_j\sigma^z_k
%\end{equation}
%

%\begin{equation}
%    H_{C3}= \sum_{j<k<m} c_{jkm} \sigma^z_j\sigma^z_k\sigma^z_m
%\end{equation}

%\begin{equation}
%    H_{C3}= \sum_{j<k<m<n} c_{jkmn} \sigma^z_j\sigma^z_k\sigma^z_m\sigma^z_n
%\end{equation}


==> 2__Methods.tex <==
\section{Methods}
In this paper, we use two kinds of binary variables, which are a Boolean variable whose value is either $0$ or $1$ and a spin variable whose value is either $-1$ or $+1$. The value of $0$ in the Boolean variable will be mapped to $+1$ in the spin variable and vice versa, whereas $1$ of the Boolean's will be mapped into $-1$ in the spin variable and vice versa. 
 As an example, a (Boolean) bit string such as $010110$ is mapped into a (spin) vector $[1, -1, 1, -1, -1, 1]$. Both of the Boolean and spin variables will be used interchangeably according to the context of discussion.
\input{2_1__HSEARCH}
\input{2_2__QAOA_HSEARCH}
%\input{2_2__QAOA_General}
%\input{2_3__QC_kbody}
%\input{2_4__QAOA_HSEARCH}


==> 3_0_Intro_2_Experiments.tex <==
We conducted experiments using both simulators and quantum hardware. In the latter case, we implemented a simple experiment on an IBM quantum computer. Before implementing the quantum circuit for the Hadamard search, which involves several $k$-body interaction terms, we tested its elementary circuits shown in Fig. \ref{FIG_1BODY} individually. The performance of each circuit met expectations, with the solution distributions confirming the circuit's validity. Detailed results are provided in the Supplementary Information.

%We do the experiments using both of simulators and quantum hardware. In the latest case, we implement a simple experiment on low qubit number of IBM quantum computer. Before implementing the quantum circuit in Hadamard search, which involves several k-body interaction terms, we have tested its elementary circuits displayed in Fig.\ref{FIG_1BODY} individually. The performance for each of these circuits are as expected, i.e., the distribution of solutions shows the validity of the circuit. Detail of the results can be found in the Supplementary Information.

==> 3_1_Performance_Metric.tex <==
%\subsection{Performance Metrics}
%In general, the output of the algorithms discussed in this paper will be $L$-length bit strings, so that there will be $2^L$ possible combination of bit strings to check its correctness or validity.

The outputs of the algorithms discussed in this paper are $L$-length bit strings, resulting in $2^L$ possible combinations. An output string is considered valid or correct if the value of the associated non-negative error or energy function—such as the Williamson or Turyn cost function—is zero. Otherwise, it is labeled as incorrect (wrong). To evaluate the algorithm's performance in producing correct solutions, we compare it to an algorithm that randomly generates all possible $L$-length bit strings. Accordingly, we introduce the xRAR (\emph{x-Algorithm to Random-Algorithm Ratio}) as a performance metric for a given x-algorithm.

%The outputs of the algorithms discussed in this paper are in the form of $L$-length bit strings, so that there are $2^L$ possible combination of them. A result (an output string) is labelled as valid or correct when the value of the non-negative error/energy function related to the algorithm, i.e. the value of the Williamson or Turyn cost function,  is equal to zero. Otherwise, it is labelled as wrong. To measure the performance of the algorithm in producing correct solutions, we can compare it to an algorithm that randomly generate every possible combination of an $L$ length bit string. Therefore, for a given x-algorithm to measure, we propose xRAR (\emph{x-Algorithm to Random-Algorithm Ratio}) as a performance metric. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.95\columnwidth] {img/qaoa_flow_n_xrar_def}
    \caption{Workflow diagram and performance metric: (a) Performance Measure in Term of xRAR. The probability $P_x$ of correct or valid answers of the x-algorithm that generates $L$-length bit strings is compared to $P_R$, which is the correct probability of a random algorithm that generates $L$-length (uniform) randomly distributed bit strings., (b) The QAOA processing steps.}
    \label{FIG_experiment_flow} %FIG_perf_XRAR
\end{figure}
%%
%{img/XRAR_definition.jpg} %{img/QRAR_definition.jpg}
%\caption{Performance Measure in Term of xRAR. The probability $P_x$ of correct or valid answers of the x-algorithm that generates $L$-length bit strings is compared to $P_R$, which is the correct probability of a random algorithm that generates $L$-length (uniform) randomly distributed bit strings.} %When $P_x > P_R$, then the x-algorithm is considered useful.}

The random algorithm generates $2^L$ number of bit strings and we can evaluate whether each of the bit string is valid or not. If there are $S_R$ valid solutions among the $2^L$ random bit strings and we assume a uniform probability distribution, the probability of finding a valid solution, $P_R$, is given by $P_R = \frac{S_R}{2^L}$. Similarly, the solutions generated by a quantum circuit that represents the x-algorithm are also probabilistic, and we can calculate the probability $P_x$ of valid solution of the x-algorithm. Therefore, the value of xRAR; which conceptually is illustrated by Fig.\ref{FIG_experiment_flow} (a), is given as follows

%(Note that other algorithm, such as simulated annealing, also can be measured similarly)
\begin{equation}
    xRAR = \frac{P_x}{P_R}
    \label{EQ_XRAR}
\end{equation}
%
The value of xRAR in Eq. (\ref{EQ_XRAR}) is a positive real number. An xRAR value where $0 < \textit{xRAR} < 1$ indicates that the x-algorithm performs worse than the random algorithm $R$, $\textit{xRAR} = 1$ signifies comparable performance to the random algorithm, and $\textit{xRAR} > 1$ suggests that the x-algorithm outperforms the random algorithm $R$.

The execution steps of the QAOA used in the experiments are shown in Fig. \ref{FIG_experiment_flow} (b). When running the quantum algorithm, either on a simulator or a real quantum computer, we repeat the process $N$ times, referred to as the number of shots. This produces $N$ solutions or bit strings, each with a corresponding energy or error. A specific part of the algorithm computes the average or expectation value, allowing us to determine whether any of the bit strings achieve the minimum energy, as indicated in the \emph{Extraction of Measured Qubits} block in the figure. We can count the number of valid solutions at each iteration step and also after reaching the lowest average energy for a given experimental setup. The number of correct solutions is then used to evaluate the algorithm's performance.

%The execution steps of the QAOA in the experiments is displayed in  Fig.\ref{FIG_experiment_flow} (b). When running the quantum algorithm, either in a simulator or in a real quantum computer, we repeat the run $N$ times, which is called as the number of shots. It yields $N$ number of solutions/ bit strings and its corresponding energy/error. A particular block/part of the algorithm will calculate the average or expectation, where we also can check whether particular bit strings or solution achieve a minimum energy shown as the block \emph{Extraction of Measured Qubits} in the figure. We can count the number of the valid solution in each iteration step and after the lowest average energy for a particular experiment setup is achieved. The number of correct solutions can be used for determining the performance of the algorithm.

In addition to xRAR, we also evaluate the performance of the algorithm using an error metric. This error metric is defined as the accumulated or total objective values of all generated solutions, with the objectives measured by either the Williamson or Turyn cost functions, as given by Eq. (\ref{EQ_cost_williamson}) and Eq. (\ref{EQ_cost_turyn}), respectively. The error is normalized by the maximum value of each cost function and then compared to the value obtained by a random algorithm through exhaustive search.

For a particular order of H-SEARCH that generates $N_Q$-length bit string solutions with a maximum objective error of $E_{max}$ and a total error for all possible $2^{N_Q}$ bit strings equal to $E_{tot}$, the normalization factor is $2^{N_Q}E_{max}$. The average error is given by $E_{tot}/2^{N_Q}$, and the normalized average error is $E_{tot}/(2^{N_Q} E_{max})$. This normalized average error is used to compare the performance of algorithms with varying numbers of shots (samples).

%In addition to XRAR, we also evaluate the performance of the algorithm with an error metric. This error metric is the accumulated or total objective values of all generated solutions, with the objective measure are given by either the Williamson or Turyn cost functions given by Eq.(\ref{EQ_cost_williamson}) and Eq.(\ref{EQ_cost_turyn}), respectively. The value is normalized by the maximum value of each cost function, then compared to the value of random algorithm which is calculated by exhaustive search. Therefore, for a particular order of H-SEARCH that generates $N_Q$-length bit string solution with maximum objective error of $E_{max}$ and total error for all possible $2^{N_Q}$-bit string equal to $E_{tot}$, we have normalization factor $2^{N_Q}E_{max}$, the average error of $E_{tot}/2^{N_Q}$, and normalized average error of $E_{tot}/(2^{N_Q} E_{max})$. The normalized average error is used to compare the performance of algorithms with various number of shots (sampling).
%\begin{equation}
%    \nonumber
%    C=E_{max} 2^{NQ}
%\end{equation}

%when an x-algorithm executed $N_x$ times (number of shots) has total error of $E_x$, whereas corresponding random algorithm generated $N_Q$-length bit string has maximum objective error of $E_{R}$

==> 3_2_HSEARCH_Williamson.tex <==
%//////// comparison of energy landscape /////////////
%/// PEL: Potential Energy Landscape
% williamson
% ------
% >>> 12 --> NQ = 5
% > 20 --> NQ = 9
% >>>> 28 --> NQ = 13
% turyn
% ------
% >>> 44 --> NQ = 16-11 = 5
% >>> 68 --> NQ = 24-11 = 13
%\newpage
%\subsection{The QAOA Williamson/Baumert-Hall Method}
%\subsubsection{Lowest Order Matrix}
The lowest order case for the Williamson method is 12, which corresponds to 36-order Baumert-Hall H-matrix, requires 8 qubits to implement. The energy function of this problems was obtained similarly to our previous paper \cite{suksmono_2022}. 
%The energy function of this problems, in terms of spin variables $s_i$, is obtained similarly to our previous paper [suksmono, minato]. , which is given as follows
%--
%\begin{equation}
%  \begin{split}
%    E_k(s)= 2s_0s_1 + 2s_2s_3 + 2s_4s_5 + 2s_6s_7 + s_0s_1s_2s_3 + s_0s_1s_4s_5 \\
%    + s_0s_1s_6s_7 + s_2s_3s_4s_5 + s_2s_3s_6s_7 + s_4s_5s_6s_7 + 4
%  \end{split}
%  \label{EQ_E_williamson_12}
%\end{equation}
%
%in Eq.(\ref{EQ_H_williamson_12})

%% -- PEL 12-Williamson vs &44 ------
\begin{figure*}[t]
    \centering
    {{\includegraphics[width=0.90\columnwidth]
    {img/PEL_W12_vs_T44} }} %
    \caption{Comparisons of lowest order PEL (Potential Energy Landscape): (a) 12-order QAOA-Williamson and (b) 44-order QAOA-Turyn}%
    \label{FIG_WBH_QC}%
\end{figure*}
%
An exhaustive search to all possible $2^{8}$ bit strings that yields minimum energy; and therefore correct bit strings, found $64$ WBH-sequences as valid solutions. This result yields the probability value to find the solution of 8-length uniformly distributed bit strings $P_R=\frac{1}{4}$; therefore, the maximum QRAR performance is $\frac{1}{P_R} = 4$. It is also found that the maximum value of the cost function is $18$ and the total error of $1,024$; implying that the normalized average error is equal to $0.2222$. The Hamiltonian of this problem is given by 
%--
\begin{equation}
  \begin{split}
    \hat{H}\left( \hat{\sigma}\right)=2 \hat{\sigma}^z_0\hat{\sigma}^z_1 + 2\hat{\sigma}^z_2\hat{\sigma}^z_13 + 2\hat{\sigma}^z_4\hat{\sigma}^z_5 + 2\hat{\sigma}^z_6\hat{\sigma}^z_7 %\\
    + \hat{\sigma}^z_0\hat{\sigma}^z_1\hat{\sigma}^z_2\hat{\sigma}^z_3 + \hat{\sigma}^z_0\hat{\sigma}^z_1\hat{\sigma}^z_4\hat{\sigma}^z_5 + \\ \hat{\sigma}^z_0\hat{\sigma}^z_1\hat{\sigma}^z_6\hat{\sigma}^z_7 
    + \hat{\sigma}^z_2\hat{\sigma}^z_3\hat{\sigma}^z_4\hat{\sigma}^z_5 + \hat{\sigma}^z_2\hat{\sigma}^z_3\hat{\sigma}^z_6\hat{\sigma}^z_7 +  \hat{\sigma}^z_4\hat{\sigma}^z_5\hat{\sigma}^z_6\hat{\sigma}^z_7 %\\
    + 4
  \end{split}
  \label{EQ_H_williamson_12}
\end{equation}
%
Note that in the minimization, the constant term can be dropped without affecting the result. We will perform some experiments for this case with both of the simulator and the real quantum computer.
%in Eq.(\ref{EQ_H_williamson_12})

%% -- 12-Williamson/36-Baumert Hall ------
%\begin{figure*}[t]
%    \centering
%    {{\includegraphics[width=0.8\columnwidth]
%    {img/qc_williamson_12.jpg} }} %
%    \caption{Quantum circuits 12-Williamson/36-Baumert Hall QAOA Method}%
%    \label{FIG_WBH_QC}%
%\end{figure*}
%

First, we run the QAOA-HSEARCH algorithm in a quantum computer simulator (IBM-Qiskit) with various number of layers, random initialization of $\{\beta_0, \gamma_0\}$ parameters, and using COBYLA (Constrained Optimization BY Linear Approximation) which is available in the Python library for optimization \cite{powell_2012}.  Figure \ref{FIG_1BODY} (d) shows a one-layer quantum circuit related to Eq.(\ref{EQ_H_williamson_12}).%, while the experiment results is displayed in Fig.\ref{FIG_WBH} (a). %and a table in Fig.\ref{FIG_SIM_vs_QPU}.

% -- 12-Williamson/36-Baumert Hall ------
\begin{figure*}[t]
    \centering
    \subfloat[\centering Simulation]
    {{\includegraphics[width=0.50\columnwidth]{img/perf_williamson_12_SIM.jpg} }} %
    %\hspace{2 cm}
    %\\
    \subfloat[\centering Hardware]
    {{\includegraphics[width=0.50\columnwidth]{img/perf_williamson_12_QPU.jpg} }} %
    %\hspace{1}   
    \caption{Performance of 12-Williamson/36-Baumert Hall QAOA Methods. Fig. (a) displays simulation results: solid blue line with blue circles is the XRAR, solid blue line is the upper bound of XRAR which is equal to 4, red-dotted line with circle is the normalized objective error, dotted line is the lower bound of error which is equal to zero. Fig. (b) Shows the hardware performance: dotted blue line with $\times$ symbols is the objective error, dotted blue line at the upper part is the error threshold for random algorithm, solid red line with circle is the mean XRAR, solid red line is the XRAR of random algorithm, and the red dashed-dot with $\times$ symbols are maximum value of XRAR at corresponding layer number}%
    \label{FIG_WBH}%
\end{figure*}

The energy distribution as a function of $\gamma$ and $\beta$ parameters displayed as PEL (Potential Energy Landscape) in Fig.\ref{FIG_WBH_QC} shows a periodic landscape, with minima located around the first (right upper part) and third quadrants (left lower part). Fig.\ref{FIG_WBH} (a) shows the performance of the algorithm with the number of layers $p$ are increased stepped wisely, i.e, $ p = 1, \frac{NQ}{2}, NQ, 2NQ, 4NQ$. Considering the location of the minima which are indicated in the PEL, the initialization of the parameters have been picked up within $(-0.5, 0.5)$ interval. We repeat the experiment 10 times and plot the mean value of XRAR and Error in the figure. We observed that the value of xRAR consistently increased asymptotically to its maximum theoretical value of $XRAR=4$ at $p=4NQ=32$. At the same time, we observed that increasing the number of layer reduces the error. The resulting 12-order of the Williamson's and its corresponding 36 order of Baumert-Hall's are displayed in Fig. \ref{FIG_WBH_mtx} (a) and Fig. \ref{FIG_WBH_mtx} (b), respectively.  
%
%We repeat the experiment 7 times and plot the mean value of xRAR and objective function/error in the graph. We observed that the value of xRAR consistently increased to about $3.92$ at $p=4NQ=32$, which approaches the maximum theoretical value of $4$. At the same time, the objective error tend to decrease with the increasing number of layers. The resulting 12-order of the Williamson's and its corresponding 36 order of Baumert-Hall's are displayed in Fig. \ref{FIG_WBH} (a) and Fig. \ref{FIG_WBH} (b), respectively.  
% ******* ANALYSIS *****
%This results is in accordance with the predictions; in the sense that increasing the number of Trotter's layers improve the approximation and therefore the xRAR approach theoretical value, whereas the error decreased to zero. This is an ideal case, which only occors when we have a perfect errorles/free-noise qubits. 

%% -- 12-Williamson/36-Baumert Hall ------
%\begin{figure*}[t]
%    \centering
%    %\subfloat[\centering Performance: Simulator vs QPU]
%    {{\includegraphics[width=1.0\columnwidth]{img/williamson_12_sim_vs_qpu.jpg} }} %
%    \caption{ Comparison of Simulator and Quantum Hardware Performance of 12-Williamson/36-Baumert Hall QAOA Methods}%
%    \label{FIG_SIM_vs_QPU}%
%\end{figure*}

We also implemented the algorithm of finding 12-order Williamson matrix in a quantum computer hardware.  An IBM quantum computer, in this case is the IBM-Brisbane machine powered by a 127 qubits Eagle r.3 of version 1.1.6 quantum processor, was employed. The processor's qubits mean coherence time are $T_1 \approx 227 \mu s, T_2 \approx  130 \mu s$ with median ECR error $ \approx 7 \times 10^{-3}$ and median SX error  $ \approx 2 \times 10^{-4}$. We also repeat the run 10 times and the number of shots in the hardware is set to 1024. The results is displayed in Fig. \ref{FIG_WBH}(b), which is the quantum hardware (QPU) performance for the QAOA 12-order Williamson method with number of layers $1, 2, 3$ and $4$. This figure shows that although the mean error of QAOA implemented on hardware (blue dotted line with "$\times$" symbols) are consistently lower than the mean error of random algorithm (blue dotted line in the upmost part), the mean XRAR performance (red solid line with red circle symbols) is sometimes only slightly better than the random algorithm bound (red solid line) for number of layer of 1 and 3, and worse for 2 and 4. Since initialization of the angle can influence the final results, in term of XRAR, we also display the maximum XRAR for each repeated 10 times run. The max RAR performance initially higher than random but then tend to decrease when the number of layers are increased. This shows the circuit depth increases the noise level of the qubits.  

% Whereas in the simulation we repeat the experiment a number of time by initializing random seed at various values, due to a more limited resource, the experiments with the quantum hardware is only performed once to each number of layers. We select the random seed that yields the maximum number of correct solution, then get the optimized $\{\gamma, \beta \}$ parameter to be implemented in the quantum hardware.
%The mean XRAR curve shows that the hardware performance is only slighty better than the random algorithm 
%This figure shows that, when the number of layer $p$ is small, the xRAR performance is slightly better than random algorithm although the error is relatively low. In contrast with the simulator with ideal qubits whose xRAR increases and approaching the ideal value of $xRAR=4$, the value of xRAR of the H/W start to deteriorate with increasing number of layers or depth of the circuit. Especially, starting from $p=16$ there is no observed improvement of the xRAR on the hardware, which indicates that the qubit error in the QPU significantly affects the performance of the QAOA algorithm.
%Comparison of simulation and real quantum hardware for various number of layers are also shown as curves in Fig.\ref{FIG_SIM_vs_QPU}.

% In the experiments, after running the simulator at various values of initial random seeds, we chose the seed that yields maximum number of valid solution, then implement the quantum circuit with the optimized $\{\gamma, \beta\}$ parameters in the QPU. 
%In the simulation, we repeat the experiment multiple times with initial values of $\{\gamma, \beta\}$ initialized randomly within--considering the location of the apparent minima, the interval of $(-0.5, 0.5)$.

% -- 12-Williamson/36-Baumert Hall ------
\begin{figure*}[h!]
    \centering
    \subfloat[\centering 12-order Williamson H-matrix]
    {{\includegraphics[width=0.3\columnwidth]{img/mtx_williamson_H_12.jpg} }}%
    \hspace{2 cm}
    \subfloat[\centering 36-order Baumert-Hall H-matrix]
    {{\includegraphics[width=0.3\columnwidth]{img/mtx_bhall_H_36.jpg} }}%
    %{{\includegraphics[width=0.6\columnwidth]{img/had_baumerthall_36.jpg} }}%
    %\\
    \caption{The 12-order Williamson and 36-order Baumert-Hall Hadamard Matrices found by the proposed algorithms. Both simulation and hardware found identical H-matrices. In the figure, white boxes represent "+1" elements and the black ones represent "-1".}%
    \label{FIG_WBH_mtx}% 
\end{figure*}
%
%Results when running the circuit into quantum simulator is shown in Fig. \ref{FIG_WBH} (b). The highest histogram indicates the solution, in this case is a kind of sequence to generate $\{A,B,C,D\}$ submatrices for constructiong the Williamson and Baumert-Hall matrix. 



==> 3_3_HSEARCH_Turyn.tex <==
%\newpage
%\subsection{The QAOA Turyn Method}
In the Turyn-based method, for a particular order of H-matrix that we want to construct, we have to find a corresponding TT (Turyn Type)-Sequence \cite{turyn_1974, kharaghani_rezaie_2004, london_2013, suksmono_2022}. In term of previously formulated energy function in Eq.(\ref{EQ_cost_turyn}), we are looking for a T-string $\vec{s}$. For even positive integers $N=4, 6, 8, ... $, the order of related Turyn's Hadamard matrix will be $M=4(3N-1)$ and the number of variables or required qubits is $Q=4N-11$. We will do experiments for $N=4, 6, 8$ that corresponds to order $M=44, 68, 92$ which requires $Q=5, 13, 21$ qubits.

%% -- Turyn-44 >> 5 qubits ------
%\begin{figure*}[h!]
%    \centering
%    \subfloat[\centering QAOA circuit for finding 44-order Hadamard matrix Using Turyn Method]
%    {{\includegraphics[width=0.80\columnwidth]{img/qc_h44_1_layer.jpg} }}%
%    \caption{Results for 44-order Turyn Method}%
%    \label{FIG_QC_turyn_44}%
%\end{figure*}

In the first experiment, we want to find a Turyn H-matrix of order-44 which needs 5 qubits. The problem Hamiltonian is given by the following expression,
%The energy function is given by the following,
%
%\begin{equation}
%  \label{Es_44_Turyn}
%  \begin{split}
%    \hat{H}\left( \hat{\sigma}\right)=s_0s_1s_2 + s_0s_3s_4 + s_0s_3 - s_0s_4 + s_1s_2s_3s_4 \\
%    + s_1s_2s_3 + 2s_1s_2 + s_1s_3s_4 + s_1s_3 + s_1s_4 + s_1 + s_2s_3s_4 \\
%    + s_2s_3 + s_2s_4 + s_2 + s_4 + 5
%    \end{split}
%\end{equation}
%
%and its corresponding Hamiltonian is given by,

\begin{equation}
  \label{Hs_44_Turyn}
  \begin{split}
    \hat{H}\left( \hat{\sigma}\right)=\hat{\sigma}^z_0\hat{\sigma}^z_1\hat{\sigma}^z_2 + \hat{\sigma}^z_0\hat{\sigma}^z_3\hat{\sigma}^z_4 + \hat{\sigma}^z_0\hat{\sigma}^z_3 - \hat{\sigma}^z_0\hat{\sigma}^z_4 + \hat{\sigma}^z_1\hat{\sigma}^z_2\hat{\sigma}^z_3\hat{\sigma}^z_4 \\
    + \hat{\sigma}^z_1\hat{\sigma}^z_2\hat{\sigma}^z_3 + 2\hat{\sigma}^z_1\hat{\sigma}^z_2 + \hat{\sigma}^z_1\hat{\sigma}^z_3\hat{\sigma}^z_4 + \hat{\sigma}^z_1\hat{\sigma}^z_3 + \hat{\sigma}^z_1\hat{\sigma}^z_4 + \hat{\sigma}^z_1 + \hat{\sigma}^z_2\hat{\sigma}^z_3\hat{\sigma}^z_4 \\
    + \hat{\sigma}^z_2\hat{\sigma}^z_3 + \hat{\sigma}^z_2\hat{\sigma}^z_4 + \hat{\sigma}^z_2 + \hat{\sigma}^z_4 + 5
    \end{split}
\end{equation}
%
%The corresponding quantum circuit can be constructed automatically using a construction algorithm, whose one layer circuit is shown in Fig. \ref{FIG_1BODY} (f). We then run the QAOA on both of quantum simulator and quantum hardware, which successfully found the 44-order Turyn H-matrix. 
%
The corresponding quantum circuit can be automatically constructed using a construction algorithm, with a single-layer circuit depicted in Fig. \ref{FIG_1BODY} (f). We then ran the QAOA on both a quantum simulator and quantum hardware, successfully identifying the 44th-order Turyn H-matrix. As shown in the QAOA flowchart in Fig. \ref{FIG_experiment_flow}, normally we need to put the process done in the quantum computing inside the optimization, requiring exclusive access to the device. However, since we used a public access to a 5 qubits IBM quantum computer, such dedicated access was not permitted. Therefore, we only implemented the optimized quantum circuits obtained in the simulation into the 5 qubits IBM Quito.

\begin{figure*}[h!]
    \centering
    \subfloat[\centering histogram of IBM Quito]
    {{\includegraphics[width=0.6\columnwidth]{img/h_44_ibm_quito.jpg} }}%
    %
    \subfloat[\centering 44-order Turyn H-matrix]
    {{\includegraphics[width=0.35\columnwidth]{img/mtx_turyn_44.jpg} }}%
    \caption{Results for 44-order Turyn method: (a) Histogram of the output when running the algorithm in IBM Quito. The inset shows qubit configuration on the quantum device. (b) A Turyn Hadamard matrix of order-44 found by the proposed method running on IBM Quito}%
    \label{FIG_turyn_44}%
\end{figure*}

The obtained 44-order H matrix for both of the simulator and hardware are identical, which is shown in Fig. \ref{FIG_turyn_44}: (a) output histogram of implemented algorithm in IBM-Quito, and (b) result of order-44 of the Turyn H-matrix. The histogram in Fig. \ref{FIG_turyn_44} (a) indicates that the number of the valid solution, i.e. the bit string "11100", is equal to 11; which means that it consists of about $6 \%$ valid solution. Since random algorithm would have yield only $3.1 \%$, the quantum processor indicates a slight advantage over the classical one.


==> 3_4_HSEARCH_Higher_Order_Matrices.tex <==
%\subsection{Finding Higher-order H-matrices}
The PEL of the QAOA for higher-order H-matrices is more irregular compared to that for lower-order matrices, as shown previously. This suggests that selecting initial parameters is both challenging and crucial. In the followings, we show the results of finding 44-order Williamson/132-order Baumert-Hall matrices using a simulator. We used a single-layer QAOA and experimented with various initial parameters, selecting the best-performing configuration. The required number of qubits to implement this scheme is 24. After setting the number of sampling to 10,000 shots, we obtained the mean xRAR on 10 different parameter initialization is equal to 1.14 with the maximum value of 3.50. One of the obtained matrix is displayed in Fig. \ref{FIG_WBH_44_132}, where (a) shows 44-order Williamson and (b) the 132-order Baumert-hall matrices.

% -- williamson/baumert-hall: 12 ~ 44 ------
\begin{figure*}[h!]
    \centering
    \subfloat[\centering 44-order Williamson Hadamard matrix]
    {{\includegraphics[width=0.45\columnwidth]{img/mtx_williamson_H_44.jpg} }}%
    %
    \subfloat[\centering 132-order Baumert-Hall Hadamard matrix]
    %{{\includegraphics[width=0.45\columnwidth]{img/mtx_bhall_D_132.jpg} }}%
    {{\includegraphics[width=0.45\columnwidth]{img/mtx_bhall_H_132.jpg} }}%
    \caption{Experiment Results of Simulator and Quantum Hardware: (a) Williamson Matrix of Order 44 and (b) Baumert-Hall of Order 132}%
    \label{FIG_WBH_44_132}%
\end{figure*}
%%%


==> 3__Experiments.tex <==
\section{Experiments}
%%
\input{3_0_Intro_2_Experiments}
\input{3_1_Performance_Metric}
\input{3_2_HSEARCH_Williamson}
\input{3_3_HSEARCH_Turyn}
\input{3_4_HSEARCH_Higher_Order_Matrices}


==> 4__Discussions.tex <==
\section{Discussion}
%We have shown a possibility to implement a Hadamard matrix searching algorithm into a circuit-based quantum computer; both on a simulator and a real quantum device. In the framework of quantum optimization, we employed QAOA algorithm to implement the Hamiltonian of the optimization methods; which are obtained previously \cite{suksmono_2022}, into quantum circuits and run them on the circuit-based quantum computers. Although the quantum hardware only used in the lowest order case; due to limitation of the hardware access and current state of noisy qubits, the quantum simulator can found a relatively high order ones. 

We have demonstrated the feasibility of implementing Hadamard matrix search algorithms on a circuit-based quantum computer, both in a simulator and on actual quantum hardware. Within the framework of quantum optimization, we utilized the Quantum Approximate Optimization Algorithm (QAOA) to construct the Hamiltonian for optimization, as previously described in our work \cite{suksmono_2022}. This Hamiltonian was then implemented in quantum circuits and executed on circuit-based quantum computers. Due to hardware limitations and the current state of noisy qubits, the quantum hardware was only tested at the lowest order. However, the quantum simulator was able to successfully execute higher-order cases

Experimental results suggest that the difficulty in finding H-matrices using QAOA algorithms arises from the non-smoothness of the energy landscape (PEL), which becomes increasingly pronounced in higher-order cases. While the Turyn-based method is more qubit-efficient than the Williamson and Baumert-Hall (WBH) method, its more irregular energy landscape makes finding Turyn's solution more challenging.

Experiments with the lowest-order WBH case (as shown in Fig. \ref{FIG_WBH}) on the quantum simulator demonstrate that increasing the number of layers consistently enhances performance. This improvement is indicated by the xRAR metric, which asymptotically approaches the performance limit as the number of layers increases. However, implementing the algorithm on a real quantum device did not replicate this performance. With a single layer, the algorithm performed slightly better than a random algorithm on average, but this advantage diminished as the number of layers increased—unless only the best performance from multiple iterations was selected. However, the advantage of using more than one layer also disappears. These results suggest that increasing the number of layers on a NISQ device provides only limited benefits.

Late last year, in 2023, IBM successfully built a 1,121-qubit processor, known as the Condor quantum processor, although the issue of noise remains unresolved. More recently, quantum error correction experiments have reached the threshold for the surface code \cite{acharya_2024}. If these trends continue, it is likely that some of the currently unknown Hadamard matrices will eventually be discovered. The QAOA method would require 336 qubits to find the lowest unknown 668-order H-matrix using the Williamson method, or 157 qubits using the Turyn method. In terms of qubit numbers, this is within the reach of current technology. However, noise remains a significant obstacle to implementation. Nonetheless, it would be exciting to explore this domain further, particularly with exclusive access to a quantum device capable of running QAOA at full scale.

% Williamson
% ------
% K=3,5, 7,
% order= 4*K
% 
% K05=int(k/2)+1
% NQubits=4*K05
% ---
% k=3 -> order= 4k=12 -> k05=1+1=2 -> Nq=4*k05=8
% <<< k=order/4 -> k05= int(order/2)+1 -> Nq= 4*k05
% eg. 44-> k=11, k05=5+1=6 -> Nq=4*k05 = 24
% 668 >> k= 167->k05 = 83+1=84 ->Nq=4x84 = 336
% ----


% Turyn
% ---
% n=4,6,8,10, ...
% order M= 4(3*n-1) => 3*n-1 = M/4=> n=((M/4)+1)/3
% Nq=4n-11 
% ---
% eg.
% order M=44 => n = ( (44/4)+1 )/3 = 12/3 = 4
% Nq=4x4-11 = 16-11 = 5?
% 
% order M=668 => N = ( (668/4)+1)/3 = (167+1)/3 = 42
% Nq=4x42-11 = 157

%Experiments on the quantum computer simulator shows an exponential improvement of the QAOA-based quantum algorithm over random search algorithm. At the final stage, we have run and find a 44-order Williamson or 132-order Baumert-Hall matrices successfully.

% what we have achieved in this experiment
% WBH-method
% Turyn-method
%We have presented the quantum circuits of its corresponding Hamiltonian terms, from 1-body up to 4-body and confirm the correctness by simulation. 

==> 5_xAcknowledgements.tex <==
\section*{Acknowledgments}
This work has been supported partially by the P2MI Program of STEI-ITB and by the Blueqat Inc., Tokyo, Japan.

\section*{Competing interests}
The authors declare no competing interests.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AUTHORS CONTRIBUTION STATEMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Author contributions statement}
A.B.S formulated the theory, conducted the experiment(s), analyzed the results, and writing of the paper.

\section*{Data and Codes Availability}
All of codes and data will be provided upon direct request to the authors. Some parts of the codes will be made available for public upon publication of the manuscript.

==> org/2_2__QAOA_General.tex <==
%\subsection{A Brief on QAOA}
\subsection{QAOA Formulation of H-matrix Searching Problem}
%% Section 2.2 dan 2.3 perlu disatukan dng judul section spt di atas
%\subsection{A Brief on QAOA (Quantum Approximate Optimization Algorithm)}
%%%//////////////////////////////////////////////////
% this part of qaoa formulation/derivation
% from time-dependent schrodinger SHOULD BE
% verified with standard book/paper, such as Farhi's
%%%//////////////////////////////////////////////////
 
Present days quantum computers are categorized as NISQ (Noisy Intermediate Scale Quantum) devices, which means that the qubits are noisy and its number is not sufficiently large ($< 1000$) to realize a practical computational task \cite{preskill_2018}. To harness its present capability, various algorithms that works on the NISQ devices are developed, among others is the QAOA (Quantum Approximate Optimization Algorithm) proposed by Farhi \cite{farhi_2014}. It is a quantum algorithm to approximate the solution of a combinatorial optimization problem. 

%Recently, an important result was obtained by Kim et.al \cite{kim_2023}, where an evidence of the utility of the device without fault tolerance qubits is presented.
%---
%%%--Most recently, Kim et.al \cite{kim_2023} showed an evidence of the utility of NISQ device without fault tolerance qubits.

%The time-dependent Schroedinger Equation for a quantum system with Hamiltonian $H$ is given by
%\begin{equation}
%    i\hslash \frac{\partial \ket{\psi_t}}{\partial t} = H\ket{\psi_t}
%\end{equation}
%with a general solution
%\begin{equation}
%    \ket{\psi_t} = e^{-i\frac{Ht}{\hslash}}  \ket{\psi_0} = U(H,t)\ket{\psi_0}
%\end{equation}
%with unitary evolution given by
%\begin{equation}
%    U(H,t)=e^{-i\frac{Ht}{\hslash}}
%  \label{EQ_unitary}
%\end{equation}
%%//// tentative after this, ref to 
%// https://pennylane.ai/qml/demos/tutorial_qaoa_intro//
%
% H=H_1+H_2 + ... +H_n
% with H_i noncommutative in general. We can approximate using trotter-Suzuki decomposition formula
%\begin{equation}
% e^{H_i + H_j} \approx \left( e^{\frac{H_i}{n} e^{\frac{H_j}{n}} \right) ^n 
%    \label{EQ_trotter_suzuki}
%\end{equation}
%The unitary can be approximated with $n$-time step discretization as follows
%\begin{equation}
%    \nonumber
%    U(t, t_0) \approx U(t,t_n)U(t,t_{n-1}) \cdots U(t_1,t_0)
%\end{equation}
%and by using \ref{EQ_unitary}, we have
%\begin{equation}
%    \nonumber
%    U(t, t_0) \approx e^{-i\frac{H_n(t-t_n)}{\hslash}}
%    e^{-i\frac{H_{n-1}(t_n-t_{n-1})}{\hslash}} \cdots
%    e^{-i\frac{H_1(t_1-t_0)}{\hslash}}
%\end{equation}
%%%%%%%%%%%%%%%
%The QAOA is a quantum algorithm to approximate a solution of a combinatorial optimization problem that can work on the NISQ devices. It works as follows.

For an $N$-length bit string $\vec{b}=b_0b_1 \cdots b_{N-1}$, let $C(\vec{b})$ be a cost or objective function given by the following expression
%
\begin{equation}
    C(\vec{b}) = \sum_{n=0}^{N-1} C_n(\vec{b})
    \label{EQ_QAOA_basic}
\end{equation}
%
The value of cost function $C_n=1$ if $\vec{b}$ satisfies clause or Boolean function $C_n$ and it is $0$ otherwise. If $C$ is the maximum value of Eq. (\ref{EQ_QAOA_basic}), the approximation means that we seek for a bit string $\vec{b}$ where $C(\vec{b})$ is close to $C$.

Alternatively, we can change the Boolean variable $\vec{b}$ in Eq. (\ref{EQ_QAOA_basic}) with spin variables $\vec{s}$, and the maximization can also be changed into minimization. Therefore, we can restate the previous approximation problem that we are seeking for $\vec{s}=[s_0, s_1, \cdots, s_M]$ that minimize

\begin{equation}
    C(\vec{s}) = \sum_{m=0}^{M-1} C_m(\vec{s})
    \label{EQ_QAOA_spin}
\end{equation}

In the QAOA method, we have a Hamiltonian $H$ that consists of a \emph{problem Hamiltonian} $H_C$ and a \emph{mixer Hamiltonian} $H_B$,
%
\begin{equation}
    H = H_C + H_B
\end{equation}
%
Then, we construct a quantum circuit to perform the following unitary transform  
\begin{equation}
      U(\gamma, \beta) = e^{-i\beta_p H_B}e^{-i\gamma_n H_C} e^{-i\beta_{p-1} H_B}e^{-i\gamma_{n-1} H_C} \cdots e^{-i\beta_1 H_B}e^{-i\gamma_1 H_C}
    \label{EQ_QAOA_general}%
\end{equation}
where
\begin{equation}
  H_B=\sum_j b_j \sigma^x_j  
  \label{EQ_QAOA_driver}%
\end{equation}
and
\begin{equation}
    H_C=\sum_{j,k, \cdots,m,n} c_{jk\cdots mn} \sigma^z_j\sigma^z_k\cdots \sigma^z_m\sigma^z_n  
  \label{EQ_QAOA_problem}%
\end{equation}
%    H_C=\sum_{j,k, \cdots,m,n} c_{j,k,\cdots, m,n} \sigma^z_j\sigma^z_k\cdots \sigma^z_m\sigma^z_n  
In these equations, $b_j$ and $c_{j,k,\cdots, m,n}$ are constants, whereas $\sigma^x_j$ and $\sigma^z_j$ are the $j^{th}$ spin/Pauli matrices in $x$ and $z$-directions, respectively.

The product of $n$ Pauli matrices in the last term $\sigma_0^z\sigma_1^z \cdots \sigma_{n-1}^z$ is called $n$-body interaction terms. In the Hadamard Searching Problem (H-SEARCH), there are only up to 4-body interaction in the Hamiltonian, so that generally $H_C$ can be written as

\begin{equation}
    H_C=\sum_{j} c_j \sigma^z_j  +
    \sum_{j,k}c_{jk}\sigma^z_j\sigma^z_k +
    \sum_{j,k,m} c_{jkm} \sigma^z_j\sigma^z_k\sigma^z_m + 
    \sum_{j,k,m,n} c_{jkmn} \sigma^z_j\sigma^z_k\sigma^z_m\sigma^z_n 
  \label{EQ_QAOA_problem_hsearch}%
\end{equation}
%
In the followings, we will describe how to construct quantum circuits related to each of the $n$-body interactions. % and present an example of finding a 2-order H-matrix.

==> org/2_3__QC_kbody.tex <==
\subsection{Construction of Quantum Circuits with $n$-body Interaction}
% for 1-body, 2-body, 3-body, and 4-body interactions
 Consider a general problem Hamiltonian as expressed in Eq. (\ref{EQ_QAOA_problem_hsearch}). By using Eq.(\ref{EQ_QAOA_general}), the unitary for of a single layer problem's Hamiltonian can be expressed by
\begin{equation}
    \label{EQ_problem_h_unitary}
    U(\gamma)=\prod_{j}e^{-i\gamma c_j\sigma^z_j}
            \prod_{j,k}e^{-i\gamma c_{jk}\sigma^z_j\sigma^z_k}
            \prod_{j,k,m}e^{-i\gamma c_{jkm}\sigma^z_j\sigma^z_k\sigma^z_m}
            \prod_{j,k,m,n}e^{-i\gamma c_{jkmn}\sigma^z_j\sigma^z_k\sigma^z_m\sigma^z_n}
\end{equation}
%e^{-i\gamma H_C}=
%
% -- 1-Body ------
\begin{figure*}[h!]
    \centering
    \subfloat[\centering 1-body interaction]
    {{\includegraphics[width=0.45\columnwidth]{img/1_body.jpg} }}% 
    %\qquad
    \subfloat[\centering 2-body interaction]
    {{\includegraphics[width=0.45\columnwidth]{img/2_body.jpg} }} %
    %\hspace{1}
    \\
    %\\
    \subfloat[\centering 3-body interaction]
    {{\includegraphics[width=0.6\columnwidth]{img/3_body.jpg} }}%
    \\
    %\qquad
    \subfloat[\centering 4-body interaction]
    {{\includegraphics[width=0.8\columnwidth]{img/4_body.jpg} }}%
    %%%
    \caption{Quantum Circuits for 1-,2-,3-, and 4-body interaction terms in the Hamiltonian}%
    \label{FIG_1BODY}%
\end{figure*}
%
We can represent the exponentiation of $\sigma^z$ as a rotation in $z$-direction, $R_Z(\cdots)$, as  follows
\begin{equation}
    \nonumber
     U(\gamma) = e^{-i\gamma \sigma^z} 
     = e^{-i\gamma 
     \begin{pmatrix}
      1 & 0 \\
      0 & -1
     \end{pmatrix}
     }
     =  
     \begin{pmatrix}
      e^{-i\gamma} & 0 \\
      0 & e^{i\gamma}
     \end{pmatrix}
     = R_Z(2\gamma)
\end{equation}
%
By substitution of $\gamma' = c_j \gamma$, we  have
\begin{equation}
    \nonumber
     U(c_j\gamma)=U(\gamma') = e^{-c_j\gamma \sigma^z} = R_Z(2c_j\gamma)
\end{equation}
%
The first term of the product in Eq.(\ref{EQ_problem_h_unitary}), considering there are $N$ qubits to be rotated, can be expanded into

\begin{equation}
    \nonumber
    \prod_{j} e^{-ic_j\gamma \sigma_j^z} =  
    \begin{pmatrix}
      e^{-ic_0\gamma} & 0 \\
      0 & e^{ic_0\gamma}
    \end{pmatrix}
    \otimes
    \begin{pmatrix}
      e^{-ic_1\gamma} & 0 \\
      0 & e^{ic_1\gamma}
    \end{pmatrix}
    \otimes
    \cdots
    \otimes
    \begin{pmatrix}
      e^{-ic_{N-1}\gamma} & 0 \\
      0 & e^{ic_{N-1}\gamma}
    \end{pmatrix}
    %\label{EQ_unitary_1body_prod}
\end{equation}
or, by denoting the $Z$ rotation on qubit $n$ as $R_{Z_n(\cdots)}$, we can write
\begin{equation}
    \nonumber
    \prod_{j} e^{-ic_j\sigma_j^z} 
    = R_{Z_0}(2c_0\gamma) \otimes R_{Z_1}(2c_1\gamma) \otimes \cdots \otimes R_{Z_{N-1}}(2c_{N-1}\gamma)
    \label{EQ_unitary_1body_prod}
\end{equation}

%%%%% //// 
The products in Eq.(\ref{EQ_problem_h_unitary}) can be interpreted as a cascaded operation. Then, a 1-body terms in the Hamiltonian that is expressed by $H_{C1}= \sum_j c_j \sigma^z_j$ can be implemented as a quantum circuit given by Fig. \ref{FIG_1BODY}.(a), which is a Z-rotation of angle $2c_j\gamma$.
%\begin{equation}
%    H_{C1}= \sum_j c_j \sigma^z_j
%\end{equation}
%
Higher order terms, which are 2-,3-, and 4- body interacting terms, can also be treated similarly, but with a different elementary circuits in the cascaded block. The quantum circuits implementation of the $k$-body interactions displayed in Fig. \ref{FIG_1BODY} (b), (c), and (d) are adopted from Nielsen-Chuang \cite{nielsen_chuang_2010}, Seeley \cite{seeley_2012}, and Setia \cite{setia_2018}.

A 2-body terms in the Hamiltonian $H_{C_2}= \sum_{j<k} c_{jk}\sigma^z_j\sigma^z_k$ has a corresponding circuits given by Fig. \ref{FIG_1BODY}.(b), which is a combination of CNOT and Z-rotation gate. The 3-body terms in the Hamiltonian which is expressed by $H_{C_3}= \sum_{j<k<m} c_{jkm} \sigma^z_j\sigma^z_k\sigma^z_m$ has a corresponding circuits given by Fig. \ref{FIG_1BODY}.(c), which is a combination of CNOT and Z-rotation gate acting on 3 qubits. Finally, a 4-body terms in the Hamiltonian  $H_{C_4}= \sum_{j<k<m<n} c_{jkmn} \sigma^z_j\sigma^z_k\sigma^z_m\sigma^z_n$ has a corresponding circuits given by Fig.\ref{FIG_1BODY}.(d), which is a combination of CNOT and Z-rotation gate acting on 4 qubits.

%\begin{equation}
%    H_{C2}= \sum_{j<k} c_{jk}\sigma^z_j\sigma^z_k
%\end{equation}
%

%\begin{equation}
%    H_{C3}= \sum_{j<k<m} c_{jkm} \sigma^z_j\sigma^z_k\sigma^z_m
%\end{equation}

%\begin{equation}
%    H_{C3}= \sum_{j<k<m<n} c_{jkmn} \sigma^z_j\sigma^z_k\sigma^z_m\sigma^z_n
%\end{equation}


==> org/3_3_1_Williamson_BHall.tex <==
\newpage
\subsubsection{The QAOA Williamson and QAOA Baumert-Hall Methods}
The lowest order case for the Williamson method is 12, which corresponds to 36-order of the Baumert-Hall methods that requires 8 qubits. The energy function this problems, in terms of spin variables $s_i$, is obtained similarly with our previous paper [suksmono, minato], which is given as follows
%--
\begin{equation}
  \begin{split}
    E_k(s)=2s_0s_1 + 2s_2s_3 + 2s_4s_5 + 2s_6s_7 \\
    + s_0s_1s_2s_3 + s_0s_1s_4s_5 + s_0s_1s_6s_7 \\
    + s_2s_3s_4s_5 + s_2s_3s_6s_7 + s_4s_5s_6s_7 \\
    + 4
  \end{split}
\end{equation}
Its corresponding Hamiltonian is given by
%--
\begin{equation}
  \begin{split}
    \hat{H}\left( \hat{\sigma}\right)=2 \hat{\sigma}^z_0\hat{\sigma}^z_1 + 2\hat{\sigma}^z_2\hat{\sigma}^z_13 + 2\hat{\sigma}^z_4\hat{\sigma}^z_5 + 2\hat{\sigma}^z_6\hat{\sigma}^z_7\\
    + \hat{\sigma}^z_0\hat{\sigma}^z_1\hat{\sigma}^z_2\hat{\sigma}^z_3 + \hat{\sigma}^z_0\hat{\sigma}^z_1\hat{\sigma}^z_4\hat{\sigma}^z_5 +  \hat{\sigma}^z_0\hat{\sigma}^z_1\hat{\sigma}^z_6\hat{\sigma}^z_7 \\
    + \hat{\sigma}^z_2\hat{\sigma}^z_3\hat{\sigma}^z_4\hat{\sigma}^z_5 + \hat{\sigma}^z_2\hat{\sigma}^z_3\hat{\sigma}^z_6\hat{\sigma}^z_7 +  \hat{\sigma}^z_4\hat{\sigma}^z_5\hat{\sigma}^z_6\hat{\sigma}^z_7 \\
    + 4
  \end{split}
\end{equation}
%
An exhaustive search to all possible $2^{8}$ bit strings found $64$ WBH-seqeuence as correct solutions. This gives $P_R=\frac{1}{4}$ and the maximum xRAR performance will be $\frac{1}{P_R} = 4$.

% -- 12-Williamson/36-Baumert Hall ------
\begin{figure*}[t]
    \centering
    \subfloat[\centering QAOA circuit]
    {{\includegraphics[width=0.8\columnwidth]{img/qc_williamson_12.jpg} }}%
    %\qquad
    \\
    \subfloat[\centering Energy Landscape]
    {{\includegraphics[width=0.40\columnwidth]{img/e_landscape_williamson_12_grid_100.jpg} }} %
    %\hspace{1}
    %\\
    \subfloat[\centering Performance]
    {{\includegraphics[width=0.55\columnwidth]{img/perf_williamson_12.jpg} }} %
    %\hspace{1}   
    \caption{Quantum circuits and running results of 12-Williamson/36-Baumert Hall: statistics}%
    \label{FIG_WBH}%
\end{figure*}
%
Note that in the minimization, the constant term can be dropped without affecting the result. The implementation and running results on the quantum simulator are displayed in Fig. \ref{FIG_WBH}, with (a) displays the quantum circuit for one layer. The energy distribution as a function of $\gamma$ and $\beta$ parameters displayed in (b) shows a periodic landscape, with minima located around the first and third quadrants. In the simulation, we repeat the experiment multiple times with initial values of $\{\gamma, \beta\}$ randomly within--considering the location of the minima, the interval of $(-0.5, 0.5)$. Fig.(c) displays the performance of the algorithm with the number of layers are increased stepped wisely at $1, \frac{NQ}{2}, NQ, 2\times NQ$. We observed that the value of xRAR consistently increased to about $3.8$ at $p=2NQ=16$, which approach the maximum value of $4$. At the same time, the objective errors are decreased with increasing number of layers. 

% -- 12-Williamson/36-Baumert Hall ------
\begin{figure*}[h!]
    \centering
    \subfloat[\centering 12-order Williamson]
    {{\includegraphics[width=0.6\columnwidth]{img/had_williamson_12.jpg} }}%
    %\qquad
    \\
    \subfloat[\centering 36-order Baumert-Hall]
    {{\includegraphics[width=0.6\columnwidth]{img/had_baumerthall_36.jpg} }}%
    %\\
    \caption{Quantum circuits and running results of 12-Williamson/36-Baumert Hall: Matrices}%
    \label{FIG_WBH_2}%
\end{figure*}
%
%Results when running the circuit into quantum simulator is shown in Fig. \ref{FIG_WBH} (b). The highest histogram indicates the solution, in this case is a kind of sequence to generate $\{A,B,C,D\}$ submatrices for constructiong the Williamson and Baumert-Hall matrix. 
A 12 order of the Williamson's and 36 order of Baumert-Hall's are displayed in Fig. \ref{FIG_WBH} (c) and Fig. \ref{FIG_WBH} (d), respectively.

% -- williamson/baumert-hall: 12 ~ 44 ------
\begin{figure*}[h!]
    \centering
    \subfloat[\centering 132-order Baumert-Hall Hadamard Matrix]
    {{\includegraphics[width=0.45\columnwidth]{img/mtx_bhall_H_132.jpg} }}%
    %\qquad
    %\\
    \subfloat[\centering 132-order Baumert-Hall Check Matrix]
    {{\includegraphics[width=0.45\columnwidth]{img/mtx_bhall_D_132.jpg} }}%
    \\
    \subfloat[\centering Performance Table of QAOA-Williamson/Baumert-Hall]
    {{\includegraphics[width= 0.99\columnwidth]{img/tbl_williamson_qrar_gain_12_44.jpg} }}%

    \caption{Experiment Results: (a) Obtained Baumert Hall Matrix of Order 132, (b) Check Matrix of Order 132, (c) Performance Table}%
    \label{FIG_WBH_performance_all_order}%
\end{figure*}

The IBM Quantum Simulator capable to simulate up to 32 qubits in desktop PC. However, since high qubits number takes considerable running time, we perform simulation up to 24 qubits. Therefore, the Williamson method for order $12, 20, 28, 36$ and $44$ can be simulated. They corresponds to Baumert-Hall matrix of order $36, 60, 84, 108$ and $132$ respectively. The experiment results are displayed in Fig.\ref{FIG_WBH_performance_all_order}.  

The constructed $132$-order Baumert-Hall Hadamard matrix and its corresponding check matrix are shown in Fig.\ref{FIG_WBH_performance_all_order} (a), and (b), respectively. Performance table in Fig.\ref{FIG_WBH_performance_all_order} (c) displays order and their corresponding number qubits, total number of bit string, and number of WBH-sequence. The $8^{th}$ column; which is the performance in terms of QRAR for their corresponding order, shows exponentially increasing performance of the quantum algorithm compared to the random algorithm. This is a strong indicator of quantum advantage, although in this experiment we deals with ideal qubits without error. 


==> org/3_3_2_QAOA_Turyn.tex <==
%\newpage
\subsubsection{The QAOA Turyn Method}
In the Turyn methods, for a particular order of H-matrix that we want to construct, we have to find a corresponding TT (Turyn Type)-Sequence [Turyn, Karaghani-Tayfeh-Rezaiye, London, Suksmono-Minato]. In term of previously formulated energy function in Eq.(\ref{EQ_cost_turyn}), we seek for T-string $\vec{s}$. For even positive integers $N=4, 6, 8, ... $, then the order of related Hadamard matrix is $M=4(3N-1)$, and the number of required qubits $Q=4N-11$. We will do experiments for $N=4, 6, 8$ that corresponds to order $M=44, 68, 92$ which requires $Q=5, 13, 21$ qubits.

% -- Turyn-44 >> 5 qubits ------
\begin{figure*}[t]
    \centering
    \subfloat[\centering QAOA circuit]
    {{\includegraphics[width=0.90\columnwidth]{img/qc_h44_1_layer.jpg} }}%
    %\qquad
    \\
    \subfloat[\centering Energy Landscape  of H-44]
    {{\includegraphics[width=0.45\columnwidth]{img/e_landscape_turyn_44_grid_100.jpg} }} %
    %\hspace{1}
    %\\
    \subfloat[\centering Energy Landscape of H-68]
    {{\includegraphics[width=0.45\columnwidth]{img/e_landscape_turyn_68_grid_100.jpg} }} %
     %\hspace{1}   
    \caption{Quantum circuits and running results of 44-Order Turyn Hadamard Matrix}%
    \label{FIG_turyn_44}%
\end{figure*}
%
In the first experiment, we seek for Turyn Hadamard matrix of order-44 which needs 5 qubits. The energy function is given by,

\begin{equation}
  \label{Es_44_Turyn}
  \begin{split}
    \hat{H}\left( \hat{\sigma}\right)=s_0s_1s_2 + s_0s_3s_4 + s_0s_3 - s_0s_4 + s_1s_2s_3s_4 \\
    + s_1s_2s_3 + 2s_1s_2 + s_1s_3s_4 + s_1s_3 + s_1s_4 + s_1 + s_2s_3s_4 \\
    + s_2s_3 + s_2s_4 + s_2 + s_4 + 5
    \end{split}
\end{equation}
And its corresponding Hamiltonian is given by
\begin{equation}
  \label{Hs_44_Turyn}
  \begin{split}
    \hat{H}\left( \hat{\sigma}\right)=\hat{\sigma}^z_0\hat{\sigma}^z_1\hat{\sigma}^z_2 + \hat{\sigma}^z_0\hat{\sigma}^z_3\hat{\sigma}^z_4 + \hat{\sigma}^z_0\hat{\sigma}^z_3 - \hat{\sigma}^z_0\hat{\sigma}^z_4 + \hat{\sigma}^z_1\hat{\sigma}^z_2\hat{\sigma}^z_3\hat{\sigma}^z_4 \\
    + \hat{\sigma}^z_1\hat{\sigma}^z_2\hat{\sigma}^z_3 + 2\hat{\sigma}^z_1\hat{\sigma}^z_2 + \hat{\sigma}^z_1\hat{\sigma}^z_3\hat{\sigma}^z_4 + \hat{\sigma}^z_1\hat{\sigma}^z_3 + \hat{\sigma}^z_1\hat{\sigma}^z_4 + \hat{\sigma}^z_1 + \hat{\sigma}^z_2\hat{\sigma}^z_3\hat{\sigma}^z_4 \\
    + \hat{\sigma}^z_2\hat{\sigma}^z_3 + \hat{\sigma}^z_2\hat{\sigma}^z_4 + \hat{\sigma}^z_2 + \hat{\sigma}^z_4 + 5
    \end{split}
\end{equation}
%
The quantum circuit can be constructed automatically using a construction algorithm (is it necessary to show the algorithm?). The result for H-44 is given by Fig. \ref{FIG_QC_H44_1_LAYER}.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.6\columnwidth]{img/qc_h44_1_layer.jpg}
    \caption{Quantum circuits of 44-order Turyn Hadamard. This figure shows 1 layer of the circuit.}%
    \label{FIG_QC_H44_1_LAYER}%
\end{figure}

==> org/5_References__OLD.tex <==
%\section*{References}
\begin{thebibliography} {9}
%
% -----------------------------------------------------------------------------
\bibitem{Nielsen_Chuang2010}
MA Nielsen and IL Chuang, 
{\em Quantum Computation and Quantum Information},
Cambridge Univ. Press, 2010.

\bibitem{Seeley}
J.T. Seeley, M.J. Richard, P.Love, 
“The Bravyi-Kitaev transformation for quantum computation of electronic structure,”
{\em arXiv: 1208.5986}

\bibitem{Setia}
K. Setia and J. D. Whitfield,
“Bravyi-Kitaev Superfast simulation of electronic structure on a quantum computer,”
{\em arXiv: 1712.00446}

\bibitem{Ronnow2014}
Rønnow, T.F., et.al.
"Defining and detecting quantum speedup",
{\em Science}, {\bf 2014}, Vol. 345, Issue 6195, pp. 420-424


\bibitem{Albash2018}
Albash, T. and Lidar, D.A
"Demonstration of a Scaling Advantage for a Quantum Annealer over Simulated Annealing",
{\em Physical Review X}, {\bf 2018}, 8, 031016.

\bibitem{suksmono2019}
Suksmono, A.B. and Minato, Y.
"Finding Hadamard matrices by a quantum annealing machine", 
{\em arXiv:1902.07890 [quant-ph], 2019.}

\bibitem{feynman1982}
Feynman, R.P.
"Simulating Physics with Computers", 
{\em International Journal of Theoretical Physics} {\bf 1982}, 21, pp. 467-488
%
\bibitem{p_ortiz2012} 
Perdomo-Ortiz, A. et al., 
"Finding low-energy conformations of lattice protein models by quantum annealing,"
{\em Scientific Reports} {\bf 2012}, Vol. 2, Art.No. 571.
%
% -----------------------------------------------------------------------------
\bibitem{perdomo2008}
Perdomo, A., Truncik, C., Tubert-Brohman, I., Rose, G. and Aspuru-Guzik,
"A. Construction of model hamiltonians for adiabatic quantum computation and its application to finding low-energy conformations of lattice protein models," 
{\em Phys. Rev. A} {\bf 2008}, 78, 012320–15.
%
\bibitem{biamonte2008}
Biamonte, J. D. 
"Nonperturbative k-body to two-body commuting conversion Hamiltonians and embedding problem instances into Ising spins,"
{\em Phys. Rev. A}, 77, 052331, May 2008
%
\bibitem{johnson2011}
Johnson, M. W. et.al.
"Quantum annealing with manufactured spins"
{\em Nature} {\em 2011}, 473, pp. 194–198
% -----------------------------------------------------------------------------
% -----------------------------------------------------------------------------
\bibitem{suksmono2018} 
Suksmono, A.B. 
"Finding a Hadamard Matrix by Simulated Quantum Annealing."
{\em Entropy} {\bf 2018}, 20(2), 141.
% -----------------------------------------------------------------------------
% **************************************************************************************
% ********************* OLD REFERENCES**********************************
% **************************************************************************************
% **************************************************************************************
\bibitem{lucas2014}
Lucas, A. 
Ising formulations of many NP problem.
{\em Frontiers in Physics} {\bf 2014}, {\em 2}, Art.5, 10.3389/fphy.2014.00005.
%

\bibitem{metropolis1953}
Metropolis, N., Rosenbluth, A.W., Rosenbluth, M.N., and Teller, A.H.
Equation of state calculations by fast computing machines.
{\em The Journal of Chemical Physics} {\bf 1953}, {\em 21}, 1087, 10.1063/1.1699114. 

\bibitem{kirkpatrick1983}
Kirkpatrick, S., Gelatt Jr., C.D., Vecchi, M.P.
Optimization by simulated annealing.
{\em Science} {\bf 1983}, {\em 220}, 671-680, 10.1126/science.220.4598.671. 

\bibitem{cerny1985}
Cerny, V.
Thermodynamical approach to the traveling salesman problem: An efficient simulation algorithm.
{\em Journal of Optimization Theory and Applications} {\bf 1985}, {\em 45}, 41–51, 10.1007/BF00940812.


\bibitem{kadowaki1988}
Kadowaki, T. and Nishimori, H.
Quantum annealing in the transverse Ising model.
{\em Phys. Rev.E} {\bf 1988}, {\em 58}, 10.1103/PhysRevE.58.5355.
%

\bibitem{santoro2002}
Santoro, G.E., Martonak, R., Tosatti, E. and Car, E.
Theory of quantum annealing of an Ising spin glass.
{\em Science} {\bf 2002}, {\em 295}, 2427-30, 10.1126/science.1068774.

\bibitem{boixo2014}
Boixo, S. et. al.
Evidence for quantum annealing with more than one hundred qubits.
{\em Nature Physics} {\bf 2014}, {\em 10}, 218–224, 10.1038/nphys2900.

\bibitem{heim2015}
Heim, B., Rønnow, T.F., Isakov, S.V. and Troyer, M.
Quantum versus classical annealing of Ising spin glasses.
{\em Science} {\bf 2015}, {\em 348}, 215-217, 10.1126/science.aaa4170.

\bibitem{ronnow2014}
Ronnow, D. et. al.
Defining and detecting quantum speedup. 
{\em Science} {\bf 2014}, {\em 345}, 420-424, 10.1126/science.1252319.

\bibitem{isakov2016}
Isakov, S.V. et. al.
Understanding Quantum Tunneling through Quantum Monte Carlo Simulation.
{\em Physical Review Letters} {\bf 2016}, {\em 117}, 180402, 10.1103/PhysRevLett.117.180402.

\bibitem{mazzola2017a}
Mazzola, G., Smelyanskiy, V.N. and Troyer, M.
Quantum Monte Carlo Tunneling from quantum chemistry to quantum annealing.
{\em Phys. Rev. B} {\bf 2017}, {\em 96}, 134305, 10.1103/PhysRevB.96.134305.

\bibitem{martonak2004}
Martonak, R., Santoro, G.E. and Tosatti, E.
Quantum annealing of the traveling-salesman problem.
{\em Phys. Rev. E} {\bf 2004}, 70, 10.1103/PhysRevE.70.057701. 

\bibitem{titiloye2011}
Titiloye, O. and Crispin, A.
Quantum annealing of the graph coloring problem.
{\em Discrete Optimization} {\bf 2011}, {\em 8}, 376-384, 10.1016/j.disopt.2010.12.001.
%

\bibitem{zick2015}
Zick, K.M., Shehab, O. and French, M.
Experimental quantum annealing: case study involving the graph isomorphism problem.
{\em Sci. Reports} {\bf 2015}, 10.1038/srep11168.
%

\bibitem{suksmono2012}
Suksmono, A.B.
Finding a Hadamard matrix by simulated annealing of spin-vectors.
{\em J. Phys.: Conf. Ser.} {\bf 2012}, {\em 856}, 10.1088/1742-6596/856/1/012012.

\bibitem{suzuki1976}
Suzuki, M.
Relationship between d-dimensional quantal spin systems and (d+1)-dimensional Ising systems: Equivalence, critical exponents and systematic approximants of the partition function and spin correlations.
{\em Progress of Theoretical Physics} {\bf 1976}, {\em 56}, 1454–1469, 10.1143/PTP.56.1454.

\bibitem{trotter1959}
Trotter, H.F.
On the product of semi-groups of operators.
{\em Proc. Amer. Math. Soc.} {\bf 1959}, {\em 10}, 545-551, 10.1090/S0002-9939-1959-0108732-6. 

\bibitem{sylvester1867}
Sylvester, J.J.
Thoughts on inverse orthogonal matrices, simultaneous sign successions, and tessellated pavements in two or more colours, with applications to Newton's Rule, ornamental tile-work, and the theory of numbers.
{\em Phil. Mag.} {\bf 1867}, {\em 34}, 461-475.

\bibitem{hadamard1893}
Hadamard, J.
Resolution d'une question relative aux determinants.
{\em Bulletin des Sciences Mathematiques} {\bf 1893}, {\em 17} 240–246. 

\bibitem{hedayat1978}
Hedayat, A. and Wallis, W.D.
Hadamard Matrices and Their Applications.
{\em The Ann. Of Statistics}, Princeton University Press, 1978, {\em 6}, 1184-1238.

\bibitem{horadam_1993}
Horadam, K.J.
Cocyclic development of designs.
{\em J. Algebraic Combin.} 
Kluwer Academic publisher, No.2, {\bf 1993},

\bibitem{horadam_1995}
Horadam, K.J. and de Launey,W.
Generation of cocyclic Hadamard matrices.
{\em Math. Appl.} 
Springer, Vol.325, {\bf 1995}

\bibitem{horadam_2000}
Horadam, K.J.
An Introduction to Cocyclic Generalised Hadamard Matrices.
{\em Discrete Applied Mathematics } 
Elsevier, No.102, {\bf 2000}

\bibitem{alvarez_2020}
Alvarez, V.; Armario, J.A. ; Falcon, M.R. ; Frau, M.D.; Gudiel, F. ; Guemes, M.B. ; Osuna, A.
On Cocyclic Hadamard Matrices over Goethals-Seifel Loops.
{\em Mathematics } 
MDPI, Vol.8, No.24, {\bf 2020}

\bibitem{avarez_2021}
Avarez, V.; Armario, J.A. ; Falcon, M.R. ; Frau, M.D.; Gudiel, F. ; Guemes, M.B. ; Osuna, A.
Hadamard Matrices with Cocyclic Core.
{\em Mathematics } 
MDPI, Vol.9, No.857, {\bf 2021}

\bibitem{horadam2007}
Horadam, K.J.
{\em Hadamard Matrices and Their Applications},
Princeton University Press, {\bf 2007}, ISBN: 9781400842902.

\bibitem{garg2007}
Garg, V.
{\em Wireless communications and networking} {\bf 2007}.
Morgan-Kaufman, ISBN: 9780123735805. 
%

\bibitem{seberry2005}
Seberry, J., Wysocki, B.J., Wysocki, T.A.
On some applications of Hadamard matrices.
{\em Metrika} {\bf 2005}, {\em 62}, 221–239, 10.1007/s00184-005-0415-y.

%\bibitem{Karaghani2005}
%H.~Kharaghani and B.~Tayfeh-Rezaie, "A Hadamard matrix of order 428," \emph{J. Combin. Designs}, 13 (2005), pp.435–440. 

\bibitem{paley1933}
Paley, R.E.A.C.
On Orthogonal Matrices.
{\em Journal of Mathematics and Physics} {\bf 1933}, {\em 12}, 311–320, 10.1002/sapm1933121311.

\bibitem{dadegoldberg1959}
Dade, E.C. and Goldberg, K.
The construction of Hadamard matrices.
{\em Michigan Math. J.} {\bf 1959}, {\em 6}, 247-250,10.1307/mmj/1028998229.

\bibitem{williamson1944}
Williamson, J.
Hadamard's determinant theorem and the sum of four squares.
{\em Duke Math. J.} {\bf 1944}, {\em 11}, 65-81, 10.1215/S0012-7094-44-01108-7.

\bibitem{bush1971a}
Bush, K.A.
Unbalanced Hadamard matrices and finite projective planes of even order.
{\em J.of Comb. Theo., Ser.A} {\bf 1971}, {\em 11}, 38-44, 10.1016/0097-3165(71)90005-7.

\bibitem{bush1971b}
Bush, K.A.
{\em Atti del Convegno di Geometria Combinatoria e sue Applicazioni} {\bf 1971}, {\em 131}, University Perugia.
%

\bibitem{wallis1976}
Wallis, J.S.
On the existence of Hadamard matrices.
{\em J. Combin. Theory A} {\bf 1976}, {\em 21}, 188–195, 10.1016/0097-3165(76)90062-5. 

\bibitem{battaglia2005}
Battaglia, D.A., Santoro, G.E., and Tosatti, E.
Optimization by quantum annealing: Lessons from hard satisfiability problems. 
{\em Physical Review E} {\bf 2005}, {\em 71}, 066707, 10.1103/PhysRevE.71.066707.

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% NEW REFERENCES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\bibitem{jiang2017}
Jiang, Z. et. al. 
Scaling analysis and instantons for thermally assisted tunneling and quantum Monte Carlo simulations.
{\em Physical Review A} {\bf 2017}, {\em 95}, 012322, 10.1103/PhysRevA.95.012322.

\bibitem{mazzola2017b}
Mazzola G. and Troyer, M.
Quantum Monte Carlo annealing with multi-spin dynamics. 
{\em Journal of Statistical Mechanics: Theory and Experiment}
{\bf 2017}, {\em 5}, 053105, 10.1088/1742-5468/aa6de1.

\bibitem{hormozi2017}
Hormozi, L., Brown, E.W., Carleo, G. and Troyer, M.
Nonstoquastic Hamiltonian and quantum annealing of an Ising spin glass. 
{\em Physical Review B} {\bf 2017}, {\em 95}, 184416, 10.1103/PhysRevB.95.184416.

\end{thebibliography}

==> org/OLD__2_4__QAOA_HSEARCH.tex <==
\subsection{Finding The H-matrices Using QAOA}
In this Sub Section, we present the QAOA methods for finding H-matrices using Williamson, Baumert-Hall, and Turyn methods. The first two methods will be presented as implementation examples. We will be more focused to the Turyn's methods since it potentially can be used to find H-matrices of unknown order, such as the order of 668, 716, 892, etc. 

The solution of the main problems in this paper is in the form of a bit string with length $L$, so that there will be $2^L$ possibilities of bit string to check. In this respect, we propose a metric called xRR (x-Algorithm to Random-Algorithm Ratio) as a performance indicator. In this case, what we mean with random-algorithm is the solution obtained by generating an $L$-length bit string randomly then check whether it is a solution or not. When we know beforehand that there are $S_R$ number of solution, assuming uniform probability of bit string generation, the probability will be
\begin{equation}
    P_R = \frac{S_R}{2^L}    
\end{equation}

On the other hand, since the solution given by a quantum circuit representing a quantum algorithm $A$ is also random, we can measure the solution probability $P_A$. Other algorithm, such as simulated annealing, also can be measured similarly. Therefore, we can calculate the xRR as follows
\begin{equation*}
    xRR = \frac{P_A}{P_R}
\end{equation*}
The xRR will be a positive real number, where $0<xRR<1$ indicates that the random algorithm $A$ outperform the proposed algorithm $A$; whereas $xRR>1$ means that the algorithm $A$ outperform random algorithm $R$.
%%%%
The running process of the QAOA in the experiments is displayed in Fig. \ref{}
\begin{figure}
    \centering
    \includegraphics[width=1.0\columnwidth]{img/experiment_flow.jpg}
    \caption{The QAOA Experiment}
    \label{FIG_experiment_flow}
\end{figure}
%%

\input{2_4_1_QC_kbody_cases}
\input{2_4_2_Williamson_BHall}
\input{2_4_3_QAOA_Turyn}

==> org/xx__2_3__Experiments.tex <==

\subsection{Experiments and Analysis}
%
The experiments presented in this paper were conducted using both simulators and quantum hardware. For the latter, we carried out the experiments on an IBM quantum computer. Before implementing the quantum circuit for the QAOA-based Hadamard search, which involves multiple $k$-body interaction terms, we first validate the elementary circuits shown in Fig.\ref{FIG_1BODY}, both individually and in combination. 

\subsubsection{Evaluation of Elementary Quantum Circuits}

The prototypical problem that we use to evaluate the individual elementary circuits is finding matrix's element(s) of a 2-order H-matrix. For cases involving the 1,2,3, and 4 unknown elements, the representative problem in finding unknown elements $s_1, s_2, s_3, s_4$ are given by the following $2\times 2$ matrices
%
\begin{equation}
    \nonumber
    \begin{pmatrix}
        1 & 1  \\
        1 & s_1
    \end{pmatrix},
    \begin{pmatrix}
        1 & s_1  \\
        1 & s_2
    \end{pmatrix},
    \begin{pmatrix}
        1 & s_1  \\
        s_2 & s_3
    \end{pmatrix},
    \begin{pmatrix}
        s_1 & s_3  \\
        s_2 & s_4
    \end{pmatrix}
\end{equation}
%
Then, for each cases, we formulate their corresponding energy functions $E(s)$ and Hamiltonians $\hat{H}(\hat{sigma})$, whose formulation has been described in our previous papers \cite{suksmono_minato_2019, suksmono_2022}. As an example, for 4 unknown elements of the latest matrix, the Hamiltonian is
%
\begin{equation}
    \nonumber
    \hat{H}\left( \hat{\sigma}\right)=2\left(1+\hat{\sigma}^z_{1}\hat{\sigma}^z_{2} \hat{\sigma}^z_{3}\hat{\sigma}^z_{4} \right) 
    \label{EQ_4body_hsearch_hamiltonian}
\end{equation}
%
This Hamiltonian involves a 4-body interaction term whose quantum circuit is given by Fig. \ref{FIG_1BODY} (d). Then, after inserting the mixing Hamiltonian, the quantum circuit for this QAOA problem is as displayed in Fig. \ref{FIG_4BODYX} (a). Execution on a quantum simulator gives the distribution of solutions  shown in Fig.\ref{FIG_4BODYX} (b). 

% -- 4-Body, QAOA ------
\begin{figure*}[h!]
    \centering
    \subfloat[\centering Realized Quantum Circuit in Qiskit]
    {{\includegraphics[width=0.55\columnwidth]{img/4_body_qc_qiskit.jpg} }} 
    %%
    \subfloat[\centering Distribution of solution]
    {{\includegraphics[width=0.40\columnwidth]{img/4_body_sim.png} }} %
    %%
    \caption{Evaluation result of elementary circuit for QAOA-based Hadamard matrix search: (a)  Implemented single layer QAOA quantum circuit for a problem with a 4-body interaction term, (b) Distribution of solution after running the circuit on a quantum computer simulator. This histogram shows that all solutions are found with almost uniform distribution}%
    \label{FIG_4BODYX}%
\end{figure*}

This case can be considered a simple non-cascaded QAOA problem that can be sufficiently solved by a single layer quantum circuit. All of the solutions displayed in the histogram; i.e. {0001, 0010, 0100, 0111, 1000, 1011, 1101, 1110), are correct. Calculating the total probability of all of the solutions yields the performance $xRAR = 1.998$; which almost reach maximum value of $xRAR=2$, for this problem. 

On the other hand, when elementary circuits are combined into a more complex one, the problem becomes more difficult to solve. For the general problem of mixed $k$-body cascaded circuits, we will consider two cases for the Hamiltonians: uniform coefficients and non-uniform coefficients.

First, we consider a Hamiltonian with uniform coefficients of the terms given as follow 
\begin{equation}
    \hat{H}\left( \hat{\sigma}\right)= \hat{\sigma}^z_{0} + \hat{\sigma}^z_{1} + \hat{\sigma}^z_{0}\hat{\sigma}^z_{1} + \hat{\sigma}^z_{1}\hat{\sigma}^z_{2} + \hat{\sigma}^z_{1}\hat{\sigma}^z_{2} \hat{\sigma}^z_{3} + \hat{\sigma}^z_{0}\hat{\sigma}^z_{1}\hat{\sigma}^z_{2} \hat{\sigma}^z_{3}-1
    \label{EQ_cascaded_uniform_coeffs}
\end{equation}
%
There are 4 correct solutions for this problem, which are  $\{0101, 0110, 1000, 1001\}$, so that $P_R=\frac{1}{4}$. We run this problem with various configuration and a number of iteration. Simulation results are shown in Fig.\ref{FIG_kbody_uniform_coeffs}. The results indicate that a single-layer QAOA circuit is insufficient to produce good outcomes, as shown by the histogram in (a). Accordingly, we increase the number of layers subsequently into $p=4, 8, 16, 32$.   The histogram in (b) shows the solution distribution for $p=32$, where some correct solutions exhibit dominant probability values, while the incorrect ones are suppressed. As shown by the curve in (c), the error decreases after more than 500 iterations of updating the angle parameters. The table in (d) indicates that increasing the number of QAOA layers consistently improves the xRAR performance.

% -- mixed k-body, uniform coeffs
\begin{figure*}[h!]
    \centering
    \subfloat[\centering Distribution of solution for $p=1$]
    {{\includegraphics[width=0.45\columnwidth]{img/k_bodies_uniform_coeffs_dist_p_1.jpg} }} 
    %
    \subfloat[\centering Distribution of solution for $p=32$]
    {{\includegraphics[width=0.45\columnwidth]{img/k_bodies_uniform_coeffs_dist_p_2NQ_sqr.jpg} }} 
    %%
    \\
    \subfloat[\centering Iteration curve for $p=32$]
    {{\includegraphics[width=0.48\columnwidth]{img/k_bodies_uniform_coeffs_iter_p_2NQ_sqr.jpg} }}%
    %\qquad    
    \subfloat[\centering Table of performance]
    %{{\includegraphics[width= 0.48\columnwidth]{img/k_bodies_uniform_coeffs_tbl.jpg} }}%
    {{ \begin{tabular}{|c|c|r|r|}
            \hline
            No & Num Layer $p$ & Obj. Error&    xRAR\\
              %&  $\pm0.05$ cm& $\pm0.05$ cm& $\pm0.05$ cm\\
            \hline
            1&  1&   1.850&   1.344\\
            \hline
            2&  4&   0.945&   2.117\\
            \hline
            3&  8&   0.337&   3.313\\
            \hline
            4&  16&   0.465&   3.121\\
            \hline
            5&  32&   0.115&   3.734\\
            \hline
       \end{tabular}
     %
     }}
    \caption{Experiment results for a mixed k-body Hamiltonian with uniform coefficients: (a) distribution of solution for $p=1$ showing both of correct and incorrect solutions with with comparable probability values, (b) distribution of solution for $p=32$, indicating that increasing the layer number improve the solution; non correct solutions are suppressed, (c) Curve showing decreasing of error by iteration and achieve convergence after more than 500 iteration, (d) performance table showing that increasing the number of layer will improve the performance, i.e, reducing objective error and increasing the xRAR.}%
    \label{FIG_kbody_uniform_coeffs}%
\end{figure*}

For the second case, we consider a more general Hamiltonian where the circuits of mixed $k$ body interactions is weighted with non-uniform coefficients as follows 
%
\begin{equation}
    \hat{H}\left( \hat{\sigma}\right)= \hat{\sigma}^z_{0} +2\hat{\sigma}^z_{1} + 3\hat{\sigma}^z_{2} + 5\hat{\sigma}^z_{0}\hat{\sigma}^z_{1} + 7\hat{\sigma}^z_{1}\hat{\sigma}^z_{2} + 11\hat{\sigma}^z_{1}\hat{\sigma}^z_{2}\hat{\sigma}^z_{3} + 13\hat{\sigma}^z_{0}\hat{\sigma}^z_{1}\hat{\sigma}^z_{2}\hat{\sigma}^z_{3}
    %\label{EQ_cascaded_non_uniform_coeffs}
\end{equation}
%
This problem only have one correct solution, which is $1100$, so that the probability of random algorithm is $P_R= 1/16$. Some of the simulation results are displayed in Fig.\ref{FIG_kbody_non_uniform_coeffs}. In part (a) and (b), We observe a re-concentration of the distribution toward the solution as the number of layers  $p$ increases. In (c), we observe error reduction by the iteration number. The performance table in (d) shows that increasing $p$ tends to improve the performance, although at some value of $p$, the performance degrades.

% -- mixed k-body, non-uniform coeffs
\begin{figure*}[h!]
    \centering
    \subfloat[\centering Distribution of solution for $p=1$]
    {{\includegraphics[width=0.45\columnwidth]{img/k_bodies_non_uniform_coeffs_dist_p_1.jpg} }} 
    %%
    \subfloat[\centering Distribution of solution for $p=32$]
    {{\includegraphics[width=0.45\columnwidth]{img/k_bodies_non_uniform_coeffs_dist_p_2NQ_sqr.jpg} }} 
    %%
    \\
    \subfloat[\centering Iteration curve for $p=32$]
    {{\includegraphics[width=0.48\columnwidth]{img/k_bodies_non_uniform_coeffs_iter_p_2NQ_sqr.jpg} }}%
    %%
    \subfloat[\centering Performance Table]
    %{{\includegraphics[width= 0.48\columnwidth]{img/k_bodies_non_uniform_coeffs_tbl.jpg} }}%
    %
    {{
    %
    \begin{tabular}{|c|c|r|r|}
            \hline
            No & Num Layer $p$ & Obj. Error&    xRAR\\
            \hline
            1&  1&   12.906&   0.938\\
            \hline
            2&  4&   10.049&   0.422\\
            \hline
            3&  8&   4.023&   5.766\\
            \hline
            4&  16&   5.275&   0.541\\
            \hline
            5&  32&   1.824&   10.172\\
            \hline
      \end{tabular}
    }}
    \caption{Experiment results for a problem Hamiltonian with uniform k-Body but non-uniform coefficients: (a) distribution of solution for a single layer; although the correct solution has a high probability, other incorrect solutions are also significantly high,(b) the distribution of solutions is improved after increasing the layer number into 32, correct solutions now has the highest probability, (c) error curve shows decreasing error value by iteration number, (d) table of performance by number of layer which shows that increasing the layer number tends improve the xRAR performance and reduce the error; but sometimes, the performance is also decreased.}%
    \label{FIG_kbody_non_uniform_coeffs}%
\end{figure*}
%  
%% >>>
In general, we can say that the performance of each individual circuit met our expectations, with the solution distributions confirming the circuit's validity. A more detailed results for other configurations are provided in the Supplementary Information.
%%<<<

%---
%% GENERATE FIGURES FROM PYTHON SOURCE
%% use Simulation Mode
% A quantum circuit representing a simple problem with shallow depth can easily find the solution. Fig. xyz shows an example of such circuit, with the Hamiltonian given by .... From the learning curve in FIg. abc, we see that the convergence is relatively easy to achieved in only a few number of iteration. This prob;em only need a single layer to solve.
% On the other hand, a more complex problem consisting of cascaded elementary circuits is more challenging. Fig. efg shows quantum circuit of such problem with Hamiltonian given by .... This Hamiltonian containe several terms of mixed n-body interactions and various coefficients. As a results, achieveing convergence is rather difficult as shown in FIg. klm; initiallya oscilates but settled after a few iterations. For this problem, we need several layers. Table pqr shows the increasin xRAR performance when the number of layers are increased.
% These results anticipates what we expect when running the QAOA for the H-Search problem, since the Hamiltonian will consisting of various n-body interacting terms.
% ----
% ..... A more detailed results are provided in the Supplementary Information.

%--- detailed discussion--
% Experiments with individual elementary circuits shows that the learning curve, shown as iteration number vs error,  .... Such simple low-depth circuit, representing simple problem, only need 1 layer to find the solution. The learning curve also shows that the optimum value is easily be achieved or the state easily brought into its minimum.
%
\subsubsection{Finding Hadamard Matrices}
\input{2_3_1_HSEARCH_Williamson}
\input{2_3_2_HSEARCH_Turyn}
\input{2_3_3_HSEARCH_Higher_Order_Matrices}

%We do the experiments using both of simulators and quantum hardware. In the latest case, we implement a simple experiment on low qubit number of IBM quantum computer. Before implementing the quantum circuit in Hadamard search, which involves several k-body interaction terms, we have tested its elementary circuits displayed in Fig.\ref{FIG_1BODY} individually. The performance for each of these circuits are as expected, i.e., the distribution of solutions shows the validity of the circuit. Detail of the results can be found in the Supplementary Information.

==> pseudo-codes/ltx_qc_from_hamiltonian.tex <==
\begin{algorithm}
 \caption{Create Quantum Circuit from Hamiltonian}
 \label{alg:qc_from_hamiltonian}
 \begin{algorithmic}
    %#---------------------------------------------------------
    %# Algorithm: create quantum circuit from Hamiltonian
    %#---------------------------------------------------------
    %# Input:  
    %#       H: hamiltonian of the problem with term H[0], H[1], ...
    %#       n_terms: number of terms in the Hamiltonian
    %#       beta, gamma: vector of parameters
    %#       n_qubits: number of qubits,
    %#       qubits: qubit[0], qubit[1], ..., qubit[n_qubits-1]  
    %#       n_layers: number of qaoa layers
    %# Output: 
    %#       qc = quantum circuit
    %#---------------------------------------------------------
   \Require H, $N_{terms}, $\beta$, $\gamma, $N_q$, qubits, $N_layers$
   \Output qc = quantum circuit
   \Comment{Prepare the quantum circuit}
    %prepare the quantum circuit
    \State $qc \gets CreateQuantumCircuit(N_q)$
    %qc<-create_quantum_circuit(n_qubits)

    %# using hadamard-gate, set qubits to equal superposition of |0> and |1>
    %for m=0 to n_qubits-1
    %    qc.qubit[m] <- hadamard(qc.qubit[m])
    %end
    
    %## construct n_layers qaoa quantum circuit
    %for m=0 to n_layers-1
    %    ## problem Hamiltonian
    %    for n=0 to n_terms-1
    %        # eg. H=x0 + 2x0*x1 + 3x0*x1*x2 -4x0*x1*x2*x3
    %        coeff = coefficients_of(H[n])   # coefficients_of(H[3]) = -4
    %        order = order_of(H[n])          # order_of(H[3]) = 4
    %        qlist = list_of_interacting_qubits(H[n]) ## list_of_variables(H[3]) = [0,1,2, 3] 
    %        case order(H[n]) of:
    %            1:  begin
    %                    qc <- qc.rz(2*coeff*gamma[m], qubit[qlist[0]])
    %                end
    %            2:  begin
    %                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
    %                    qc <- qc.rz(2*coeff*gamma[m], qubit[qlist[1]]) 
    %                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
    %                end
    %            3:  begin
    %                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
    %                    qc <- qc.cx(qubit[qlist[1]], qubit[qlist[2]])
    %                    qc <- qc.rz(2*coeff*gamma[m], qubit[qlist[2]]) 
    %                    qc <- qc.cx(qubit[qlist[1]], qubit[qlist[2]])
    %                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
    %                end
    %            4:  begin
    %                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
    %                    qc <- qc.cx(qubit[qlist[1]], qubit[qlist[2]])
    %                    qc <- qc.cx(qubit[qlist[2]], qubit[qlist[3]])
    %                    qc <- qc.rz(2*coeff*gamma[m], qubit[qlist[3]]) 
    %                    qc <- qc.cx(qubit[qlist[2]], qubit[qlist[3]])
    %                    qc <- qc.cx(qubit[qlist[1]], qubit[qlist[2]])
    %                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
    %                end
    %        end-case
    %    end-for
    %    #
    %    ## mixing Hamiltonian
    %    for k=0 to n_qubits
    %        qc.qubit[k] <- rotation_x(2*beta[m],qubit[k])
    %    end-for
    %end-for
 \end{algorithmic}
\end{algorithm}

==> pseudo-codes/qc_from_hamiltonian.tex <==
#---------------------------------------------------------
Algorithm: create quantum circuit from Hamiltonian
#---------------------------------------------------------
# Input:  
#       H: hamiltonian of the problem with term H[0], H[1], ...
#       n_terms: number of terms in the Hamiltonian
#       beta, gamma: vector of parameters
#       n_qubits: number of qubits,
#       qubits: qubit[0], qubit[1], ..., qubit[n_qubits-1]  
#       n_layers: number of qaoa layers
# Output: 
#       qc = quantum circuit
#---------------------------------------------------------

#prepare the quantum circuit
qc<-create_quantum_circuit(n_qubits)

# using hadamard-gate, set qubits to equal superposition of |0> and |1>
for m=0 to n_qubits-1
    qc.qubit[m] <- hadamard(qc.qubit[m])
end

## construct n_layers qaoa quantum circuit
for m=0 to n_layers-1
    ## problem Hamiltonian
    for n=0 to n_terms-1
        # eg. H=x0 + 2x0*x1 + 3x0*x1*x2 -4x0*x1*x2*x3
        coeff = coefficients_of(H[n])   # coefficients_of(H[3]) = -4
        order = order_of(H[n])          # order_of(H[3]) = 4
        qlist = list_of_interacting_qubits(H[n]) ## list_of_variables(H[3]) = [0,1,2, 3] 
        case order(H[n]) of:
            1: qc<-construct_1_body_interaction_circuit(coeff, gamma[m], qlist)
            2: qc<-construct_2_body_interaction_circuit(coeff, gamma[m], qlist)
            3: qc<-construct_3_body_interaction_circuit(coeff, gamma[m], qlist)
            4: qc<-construct_4_body_interaction_circuit(coeff, gamma[m], qlist)
        end-case
    end-for
    #
    ## mixing Hamiltonian
    for k=0 to n_qubits
        qc.qubit[k] <- rotation_x(2*beta[m],qubit[k])
    end-for
end-for



==> pseudo-codes/qc_from_hamiltonian_detail.tex <==
#---------------------------------------------------------
# Algorithm: create quantum circuit from Hamiltonian
#---------------------------------------------------------
# Input:  
#       H: hamiltonian of the problem with term H[0], H[1], ...
#       n_terms: number of terms in the Hamiltonian
#       beta, gamma: vector of parameters
#       n_qubits: number of qubits,
#       qubits: qubit[0], qubit[1], ..., qubit[n_qubits-1]  
#       n_layers: number of qaoa layers
# Output: 
#       qc = quantum circuit
#---------------------------------------------------------

#prepare the quantum circuit
qc<-create_quantum_circuit(n_qubits)

# using hadamard-gate, set qubits to equal superposition of |0> and |1>
for m=0 to n_qubits-1
    qc.qubit[m] <- hadamard(qc.qubit[m])
end

## construct n_layers qaoa quantum circuit
for m=0 to n_layers-1
    ## problem Hamiltonian
    for n=0 to n_terms-1
        # eg. H=x0 + 2x0*x1 + 3x0*x1*x2 -4x0*x1*x2*x3
        coeff = coefficients_of(H[n])   # coefficients_of(H[3]) = -4
        order = order_of(H[n])          # order_of(H[3]) = 4
        qlist = list_of_interacting_qubits(H[n]) ## list_of_variables(H[3]) = [0,1,2, 3] 
        case order(H[n]) of:
            1:  begin
                    qc <- qc.rz(2*coeff*gamma[m], qubit[qlist[0]])
                end
            2:  begin
                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
                    qc <- qc.rz(2*coeff*gamma[m], qubit[qlist[1]]) 
                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
                end
            3:  begin
                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
                    qc <- qc.cx(qubit[qlist[1]], qubit[qlist[2]])
                    qc <- qc.rz(2*coeff*gamma[m], qubit[qlist[2]]) 
                    qc <- qc.cx(qubit[qlist[1]], qubit[qlist[2]])
                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
                end
            4:  begin
                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
                    qc <- qc.cx(qubit[qlist[1]], qubit[qlist[2]])
                    qc <- qc.cx(qubit[qlist[2]], qubit[qlist[3]])
                    qc <- qc.rz(2*coeff*gamma[m], qubit[qlist[3]]) 
                    qc <- qc.cx(qubit[qlist[2]], qubit[qlist[3]])
                    qc <- qc.cx(qubit[qlist[1]], qubit[qlist[2]])
                    qc <- qc.cx(qubit[qlist[0]], qubit[qlist[1]])
                end
        end-case
    end-for
    #
    ## mixing Hamiltonian
    for k=0 to n_qubits
        qc.qubit[k] <- rotation_x(2*beta[m],qubit[k])
    end-for
end-for



















#////////////////////////////////////
# -- 1-body --
def U_C_1body(qc, c, gamma, qbs):
    # ---[ 2*C*gamma] --->
    # konstanta c, taruh dimana?
    qc.rz(2*c*gamma, qbs)
#
# -- 2-body --
def U_C_2body(qc, c, gamma, qbs):
    qc.cx(qbs[0], qbs[1])
    qc.rz(2*c*gamma, qbs[1])
    qc.cx(qbs[0], qbs[1])
    # no return, assume qml global

# -- 3-body --
def U_C_3body(qc, c, gamma, qbs):
    qc.cx(qbs[0], qbs[1])
    qc.cx(qbs[1], qbs[2])
    #
    qc.rz(2*c*gamma, qbs[2])
    #
    qc.cx(qbs[1], qbs[2])
    qc.cx(qbs[0], qbs[1])

# -- 4-body --
def U_C_4body(qc, c, gamma, qbs):
    qc.cx(qbs[0], qbs[1])
    qc.cx(qbs[1], qbs[2])
    qc.cx(qbs[2], qbs[3])
    #
    qc.rz(2*c*gamma, qbs[3])
    #
    qc.cx(qbs[2], qbs[3])
    qc.cx(qbs[1], qbs[2])
    qc.cx(qbs[0], qbs[1])

#--

